Maximal $\mathrm{PSL_2}$ subgroups of exceptional groups of Lie type

We study embeddings of $\mathrm{PSL}_2(p^a)$ into exceptional groups $G(p^b)$ for $G=F_4,E_6,{}^2\!E_6,E_7$, and $p$ a prime with $a,b$ positive integers. With a few possible exceptions, we prove that any almost simple group with socle $\mathrm{PSL}_2(p^a)$, that is maximal inside an almost simple exceptional group of Lie type $F_4$, $E_6$, ${}^2\!E_6$ and $E_7$, is the fixed points under the Frobenius map of a corresponding maximal closed subgroup of type $A_1$ inside the algebraic group. Together with a recent result of Burness and Testerman for $p$ the Coxeter number plus one, this proves that all maximal subgroups with socle $\mathrm{PSL}_2(p^a)$ inside these finite almost simple groups are known, with three possible exceptions ($p^a=7,8,25$ for $E_7$). In the three remaining cases we provide considerable information about a potential maximal subgroup.

==> 1intro.tex <==
\chapter{Introduction}

Classifying the maximal subgroups of a finite group is one of the most fundamental problems in the field of finite group theory. Aschbacher and Scott \cite{aschbacherscott1985} reduced the problem for all finite groups to understanding the $1$-cohomology groups $H^1(G,M)$ for all simple modules $M$ for all finite almost simple groups $G$, and classifying all maximal subgroups of almost simple groups.

This paper is a contribution towards the latter, ambitious goal. For alternating and classical groups there is in some sense no complete answer, since the dimensions of the classical groups (and degrees of the alternating groups) tend to infinity, although there is substantial work in this direction. However, for sporadic and exceptional groups there is a possibility of a complete answer being known.

For sporadic groups, a complete answer is known for all groups but the Monster, and here we concentrate on exceptional groups of Lie type. There is a classification of maximal subgroups for exceptional groups $G=G(q)$ for $G$ not of type $F_4$, $E_6$, ${}^2\!E_6$, $E_7$ and $E_8$ already (see \cite{wilsonrob} for example), and so we focus on the remaining cases. What is known in the literature so far is summarized in Chapter \ref{ch:maxsubgroups}, but broadly speaking, all maximal subgroups are known for these groups apart possibly from various almost simple maximal subgroups, and these are either a small list of simple groups that are not Lie type in defining characteristic, or if the potential maximal is Lie type in defining characteristic then what is left are groups of small rank and small field size, together with a large collection of possible subgroups $\PSL_2(p^a)$, the focus of this paper.

The following general theorem is a summary of our results, although we have much more detail about a putative maximal subgroup arising in (\ref{thmi:maind}).

\begin{theorem}\label{thm:generaltheorem} Let $p$ be a prime and $a,b\geq 1$ be integers. Let $G$ be the simple group $F_4(p^b)$, $E_6(p^b)$, ${}^2\!E_6(p^b)$ or $E_7(p^b)$, and let $H$ be a simple group $\PSL_2(p^a)$ contained in $G$. Write $\bar G$ for an almost simple group with socle $G$. If $N_{\bar G}(H)$ is an almost simple, maximal subgroup of $\bar G$, then one of the following holds:
\begin{enumerate}
\item\label{thmi:maina} $G=F_4(p^b)$ for some $p\geq 13$, $a=b$, and $N_{\bar G}(H)$ is unique up to conjugation;
\item\label{thmi:mainb} $G=E_7(p^b)$ for some $p\geq 17$, $a=b$, and $N_{\bar G}(H)$ is unique up to conjugation for $p=17$, and there are two classes for $p\geq 19$;
\item\label{thmi:mainc} $G=E_7(p^b)$ for some $p$, $a=7b$, and $N_{\bar G}(H)$ is unique up to conjugation;
\item\label{thmi:maind} $G=E_7(p^b)$, $p^a$ is one of $7,8,25$.
\end{enumerate}
In (\ref{thmi:maina}) and (\ref{thmi:mainb}), the subgroup $\PSL_2(p^a)$ arises from an $A_1$ subgroup of the algebraic group $F_4$ and $E_7$. In (\ref{thmi:mainc}), the subgroup $\PSL_2(p^a)$ arises from an $A_1^7$ subgroup of the algebraic group $E_7$. There are no known examples of maximal subgroups in (\ref{thmi:maind}).
\end{theorem}

We now give more information about what we prove for each group $G$.

\begin{theorem}\label{thm:f4} Let $p$ be a prime and $a,b\geq 1$ be integers. Let $G$ be an almost simple group with socle $F_4(p^b)$, and suppose that $H$ is a subgroup of $G$ with $F^*(H)=\PSL_2(p^a)$. If $H$ is maximal in $G$ then one of the following holds:
\begin{enumerate}
\item\label{thmi:f4a} $p^a=13$, $H=\PSL_2(13)$ and is a Serre embedding;
\item\label{thmi:f4b} $q=p^a$, $p\geq 13$, $F^*(H)=\PSL_2(q)$, and $H$ is the normalizer in $G$ of the fixed points $\bX^\sigma$ of an algebraic $A_1$ subgroup of the algebraic group $F_4$ under a Frobenius endomorphism $\sigma$.
\end{enumerate}
\end{theorem}

The definition of a Serre embedding is given formally in Definition \ref{defn:serreembedding}, but informally it is a copy of $\PSL_2(h+1)$ where $h$ is the Coxeter number of $G$ and this subgroup contains a regular unipotent element. (This subgroup is named after Serre as he constructed copies of $\PSL_2(h+1)$ (if $h+1$ is a prime) over all fields in \cite{serre1996}.) In recent work of Burness and Testerman \cite{burnesstesterman2017un}, Serre embeddings have been shown to come from algebraic $A_1$s, and so (\ref{thmi:f4a}) is a subcase of (\ref{thmi:f4b}) above. Thus Theorem \ref{thm:f4} implies Theorem \ref{thm:generaltheorem} for $G=F_4(p^b)$. Kay Magaard \cite{magaardphd} proved Theorem \ref{thm:f4} for $p\geq 5$ in his Ph.D. thesis, in addition proving that $b=1$ in (\ref{thmi:f4b}).

For $E_6$ we have a complete theorem, without relying on \cite{burnesstesterman2017un}, as we show that the Serre embedding lies in $F_4$.

\begin{theorem}\label{thm:e6} Let $p$ be a prime, $a,b\geq 1$ be integers, and let $G$ be an almost simple group with socle either $E_6(p^b)$ or ${}^2\!E_6(p^b)$. There does not exist a maximal subgroup $H$ of $G$ with $F^*(H)=\PSL_2(p^a)$.
\end{theorem}

Almost all of this theorem was obtained by Aschbacher \cite{aschbacherE6Vun} using geometric techniques, where only the case $p^a=p^b=11$ and $H$ contains a semiregular unipotent element, from class $E_6(a_1)$, is left open; here we prove the whole result again, using representation theory, and remove this final case using the Lie algebra structure of the adjoint module $L(E_6)$. Of course, Theorem \ref{thm:e6} implies Theorem \ref{thm:generaltheorem} for $G$ isomorphic to $E_6(p^b)$ and ${}^2\!E_6(p^b)$.

For $E_7$, here we have some potential exceptions. The difficult cases are the Serre embedding $p^a=19$ and $p^a=7,8,25$.

\begin{theorem}\label{thm:e7} Let $p$ be a prime and $a,b\geq 1$ be integers. Let $G$ be an almost simple group with socle $E_7(p^b)$, and suppose that $H$ is a maximal subgroup of $G$ with $F^*(H)=\PSL_2(p^a)$. One of the following holds:
\begin{enumerate}
\item\label{thmi:e7a} $p^a=7$, $p^a=8$ or $p^a=25$;
\item\label{thmi:e7b} $p^a=19$, $H=\PSL_2(p^a)$ and is a Serre embedding;
\item\label{thmi:e7c} $p^a=p^b$, $p\geq 17$, and $H$ is the normalizer in $G$ of the fixed points $\bX^\sigma$ of an algebraic $A_1$ subgroup of the algebraic group $E_7$. (There is one class for $p=17$, and two for $p\geq 19$.)
\item\label{thmi:e7d} $p^a=p^{7b}$ and $H$ is the normalizer in $G$ of the fixed points $\bX^\sigma$ of an algebraic $A_1^7$ subgroup of the algebraic group $E_7$.
\end{enumerate}
\end{theorem}

Again, Burness and Testerman have showed that (\ref{thmi:e7b}) is a subcase of (\ref{thmi:e7c}), and (\ref{thmi:e7d}) is the fixed points of a maximal-rank subgroup given in \cite[Table 5.1]{liebecksaxlseitz1992}. In the case (\ref{thmi:e7a}) where $p^a=8$, we can give the precise module structure of $H$ on the minimal module for $E_7$. For $p^a=7$, there are unresolved cases of potential copies of $\PSL_2(7)$ where the preimage of the subgroup in the simply connected version of $E_7$ is both $2\times \PSL_2(7)$ and $\SL_2(7)$. In both cases the module structures on both minimal and adjoint modules can be given precisely, but it seems difficult to progress further using these techniques. In the case of $p^a=25$, this is a copy of $\SL_2(25)$ inside the simply connected version of $E_7$ with the centre of the subgroup being equal to the centre of $E_7$, and we have complete information about the module structures on both the minimal and adjoint modules. If it exists, then its normalizer is a maximal subgroup of $E_7(p^b)$ for the smallest $b$ such that it embeds in $E_7(p^b)$. Theorem \ref{thm:e7} implies Theorem \ref{thm:generaltheorem} for $G$ isomorphic to $E_7(p^b)$.

We do not deal with maximal subgroups of $E_8$ here, and only consider it for certain lemmas, which will be useful in a later treatment of this case. For exceptional groups other than $E_8$, the minimal module has dimension much smaller than the dimension of the group (as an algebraic group) and we can use representation theory to analyse this module. We can still do things with the Lie algebra for $E_8$, as we did in \cite{craven2015un2}, but these are postponed to avoid making this work even longer.

\medskip

The strategy for the proofs of these theorems is given in Chapter \ref{ch:strategy}, and relies heavily on computer calculations in three ways:
\begin{enumerate}
\item The first is to compute the traces of semisimple elements of large order on various modules for exceptional groups. Tables of these traces are available for elements of small order, but we need them for very large orders, sometimes in the hundreds. For this we can use the program that Alastair Litterick produced in his Ph.D.\ thesis \cite[Chapter 7]{litterick}, or construct the normalizer of a torus explicitly in Magma and take the conjugacy classes, then compute their eigenvalues. (Litterick has produced a much faster algorithm for computing traces of elements on $p$-restricted modules, but we do not need this for our cases.)
\item The second is to do large linear algebra problems. To find all sets of composition factors that could arise as the composition factors of the restriction of a $kG$-module to a subgroup $H$ involves checking many possible combinations against the large lists of traces of semisimple elements. This is done to reduce the possible module structures for the subgroup on the minimal and adjoint modules, and was also used in \cite{litterick}.
\item The third is to construct explicit modules for finite groups, and show that certain module structures cannot exist. This would be possible by hand, at least in some cases, but incredibly complicated and prone to mistakes. In each case, a clear recipe is given for how to reproduce the module we construct to ease verifiability. The Magma commands \texttt{ProjectiveCover(M)} and \texttt{Ext(A,B)} compute projective modules and the space of extensions between two modules. If \texttt{M} is a module and \texttt{N} is a simple module, then one can construct the maximal extension of \texttt{N} by \texttt{M} with the code
\begin{verbatim}E,rho:=Ext(M,N);
Mnew:=MaximalExtension(M,N,E,rho);
\end{verbatim}
This can be used to easily verify statements made in the paper about the structures of certain modules.
\end{enumerate}
With these three uses of a computer in mind, the rest of the argument is done by hand, in Chapters \ref{ch:f4} to \ref{ch:e7oddsl}.

The structure of this article is as follows: in the next chapter we give notation and some preliminary results. In Chapter \ref{ch:maxsubgroups} we give information about maximal subgroups of finite and algebraic exceptional groups. Chapter \ref{ch:maxsubspace} gives results about how to prove results about almost simple subgroups of algebraic groups, given information about their simple socles. Chapter \ref{ch:semisimple} proves results about `blueprints', finite subgroups of an algebraic group $\bG$ that stabilize exactly the same subspaces of a (non-trivial) rational $k\bG$-module as some infinite subgroup. We obtain upper bounds on the orders of semisimple elements that are not blueprints for the minimal module for $F_4$, $E_6$ and $E_7$. In Chapter \ref{ch:unipssemis} after, we give lots of information about unipotent and semisimple elements of exceptional groups, together with information about $\slf_2$-subalgebras of exceptional Lie algebras. Chapter \ref{ch:sl2modules} gives information about modules for $\SL_2(p^a)$, and the chapter after gives some constructions of $\PSL_2$s inside $E_6$ in characteristic $3$.

We then launch into the proof proper, with Chapter \ref{ch:strategy} giving an outline of the strategy of the proof, Chapters \ref{ch:f4} and \ref{ch:e6} proving the results for $F_4$ and $E_6$, and then the three chapters after doing $E_7$ first in characteristic $2$, and then $E_7$ in odd characteristic, split into two chapters according as the embedding into the simply connected group is $2\times \PSL_2(p^a)$ or $\SL_2(p^a)$.

The first appendix gives some widely known information about the composition factors of the reductive and parabolic maximal subgroups of $F_4$, $E_6$ and $E_7$ on the minimal and adjoint modules, information that is well known but given here for ease of reference. The second gives the traces of semisimple elements of small order on the minimal and adjoint modules for the algebraic groups $F_4$, $E_6$ and $E_7$.

\bigskip

\textbf{Acknowledgement}: The author would like to thank the referee for many detailed and helpful comments that have greatly improved the exposition of the manuscript.

\endinput

==> 2notation.tex <==
\chapter{Notation and Preliminaries}
\label{ch:notation}

In this chapter we give the notation that we need, for both groups and modules, and give a few preliminary results.

Throughout this paper, $p\geq 2$ is a prime number, $q$ is a power of $p$, and $G=G(q)$ denotes an exceptional finite group of Lie type defined over $\F_q$. More specifically, let $\bG$ be a simple, simply connected algebraic group of exceptional type over the algebraic closure $k$ of $\F_p$, equipped with a Frobenius endomorphism $\sigma$, and set $G=\bG^\sigma$. The precise types of $G$ that we are interested in are those exceptional groups whose maximal subgroups are not yet known, i.e., $F_4(q)$, $E_6(q)$, ${}^2\!E_6(q)$, $E_7(q)$ and $E_8(q)$, although we do not do much in the case of $E_8(q)$, and often will exclude it from consideration.

Notice that we consider the simply connected versions of $\bG$ and $G$, so $E_7(q)$ possesses a centre when $p$ is odd, and $E_6(q)$ does for $3\mid (q-1)$. We want the simply connected versions in order to work with the minimal module and the adjoint module simultaneously. Where this is particularly important we will remind the reader, for example when considering $\PSL_2(p^a)$ embedded in the simple group of type $E_7$, where we can embed either $\SL_2(p^a)$ in $E_7$ with the centres coinciding or $2\times \PSL_2(p^a)$ into $E_7$ with the centres coinciding, representing the two possible preimages of a copy of $\PSL_2(p^a)$ in the simple group. If $G$ possesses a graph automorphism of order $2$, denote this by $\tau$; we will remind the reader of this notation when we use it.

We let $\bar G$ be an almost simple group with socle $G/Z(G)$, which embeds into $\Aut(G)$. The maximal subgroups $M$ of $\bar G$ split into three categories: $M\cap (G/Z(G))$ is a maximal subgroup of $G/Z(G)$, $M\cap (G/Z(G))$ is not a maximal subgroup of $G/Z(G)$, and $(G/Z(G))\leq M$. The third collection is easily computed, and the first can be deduced from a list of maximal subgroups of $G$ by taking normalizers. However, the second, called \emph{novelty} maximal subgroups, cannot easily be seen from the maximal subgroups of $G$. They arise in the following manner: let $H$ be a subgroup that is not maximal in a simple group $X$, but $H$ is normalized by a group of automorphisms $A$ of $X$ while every proper subgroup of $X$ properly containing $H$ is not normalized by it. In this case, $H.A$ is a maximal subgroup of $X.A$. However, it is of course very difficult to understand these if one is simply given a list of maximal subgroups of $X$, so we will prove more than simply that a given subgroup is not maximal in the simple group, but that it is contained in stabilizers of various subspaces of a given module, enough that we can see that it cannot form a novelty maximal subgroup.

Let $L(\lambda)$ denote the irreducible highest weight module of weight $\lambda$. The notation for the weight lattice is `standard', consistent with the main references in this work and can be found in for example \cite[Chapter VI]{bourbakilie2}. The modules that we normally consider are the two smallest non-trivial ones. Write $M(\bG)$ for one of the minimal modules for $\bG$, namely $L(\lambda_4)$ for $F_4$, either $L(\lambda_1)$ or $L(\lambda_6)$ for $E_6$ and ${}^2\!E_6$, $L(\lambda_7)$ for $E_7$ and not defined for $E_8$. We write $L(\bG)$ for the Lie algebra or adjoint module, which is $L(\lambda_1)$, $L(\lambda_2)$, $L(\lambda_1)$ and $L(\lambda_1)$ respectively. If $L(\bG)$ has a trivial composition factor so is not irreducible, which occurs in $E_7$ in characteristic $2$ and $E_6$ in characteristic $3$, let $L(\bG)^\circ$ denote the non-trivial composition factor, and in other cases let $L(\bG)^\circ=L(\bG)$. These two modules have the following dimensions:
\begin{center}
\begin{tabular}{ccc}
\hline Group & $\dim(M(\bG))$ & $\dim(L(\bG)^\circ)$
\\\hline $F_4$ & $26-\delta_{p,3}$ & $52$
\\ $E_6$ & $27$ & $78-\delta_{p,3}$
\\ $E_7$ & $56$ & $133-\delta_{p,2}$
\\ $E_8$ & $-$ & $248$
\\ \hline
\end{tabular}
\end{center}
In characteristic $2$, $L(F_4)$ has factors $L(\lambda_4)=M(F_4)$ and $L(\lambda_1)=M(F_4)^\tau$, where $\tau$ denotes the graph automorphism of $G$ (which does not extend `nicely' to a morphism of $\bG$, see the definition of $\Aut^+(\bG)$ in Chapter \ref{ch:maxsubgroups}), so in this case we can consider $L(\lambda_1)$ and $L(\lambda_4)$ or $L(F_4)$. In all other cases, $L(\bG)^\circ$ is irreducible.

\bigskip

We now introduce some notation for modules. All modules will be finite dimensional and are defined over $k$. If $H$ is a group, let $\Irr(H)$ denote the set of irreducible modules over the field, which is always $k$. We also write $k$ for the trivial module for any group over the field $k$, although we will also denote it by `$1$'. As usual write `$\oplus$' and `$\otimes$' for the direct sum and tensor product of two modules. Let $\Lambda^i$ and $S^i$ denote the exterior and symmetric powers.  Write $\soc^i(M)$ for the $i$th socle layer and $\rad^i(M)$ for the $i$th radical layer of $M$. Write $\topp(M)$ for the top of $M$, i.e., $M/\rad(M)$, and $\cf(M)$ for the composition factors of $M$ as a multiset. Let $H^1(H,M)$ denote the $1$-cohomology group of $M$, and in general $\Ext^1(M,M')$ denote the group of extensions with submodule $M'$ and quotient $M$. The projective cover of a module $M$ will be denoted by $P(M)$. Let $M^*$ denote the dual of $M$.

We write $M\downarrow_H$ for the restriction of $M$ to $H$. Let $H$ and $G$ be groups, let $M$ be a $kG$-module, and let $\mathcal N$ be a set of simple $kH$-modules. Write $N$ for the direct sum of all members of $\mathcal N$. The set $\mathcal N$ is \emph{conspicuous} for $M$ if, for every $p$-regular element $x$  (i.e., order not divisible by $p$) of $H$, there is a $p$-regular element $y$ of $G$ such that the eigenvalues of $x$ on $M$ coincide with the eigenvalues of $y$ on $N$. Informally, this means that $N$ could be the composition factors of $M\downarrow_H$, if $H$ were a subgroup of $G$. Normally we use this by specifying $H$ to be a subgroup of $G$, but whose composition factors on $M$ are unknown. We might not want to check all $p$-regular elements of $H$, so we will say that $\mathcal N$ is conspicuous for elements of particular orders when we do not check all elements.

If $u$ is an element of a group $H$ of $p$-power order, and $M$ is a $kH$-module, then $u$ acts on $M$ as a sum of Jordan blocks of various dimensions. If the dimensions are, say, $5$, $5$, and $1$, we write that the structure is $5^2,1$. This is in keeping with the notation from \cite{lawther1995}, which is our main reference for the actions of unipotent classes on $M(\bG)$ and $L(\bG)$. The element $u$ \emph{acts projectively} on $M$ if all blocks of $u$ on $M$ have size $o(u)$, where $o(u)$ denotes the order of $u$. This is equivalent to the restriction $M\downarrow_{\gen u}$ being a projective $k\gen{u}$-module.

We will often have to talk about the structures of modules, as in their socle layers. If $M$ is a module with socle $A$ and second socle $B$ then we can write
\[ \begin{array}{c}B\\A\end{array}\]
for this structure; however, this is often too space-consuming when we have many socle layers, and so we also write $B/A$ for this module. Generalizing this, we delineate between socle layers by `$/$', so that $A/B,C/D,E$ is a module with socle $D\oplus E$, second socle $B\oplus C$, and third socle $A$. Because of the potential for confusion with the quotient, we will always mention if we mean a quotient.

We also introduce the concepts of radical and residual. If $I$ is a subset of $\Irr(H)$, then the \emph{$I$-radical} of $M$ is the largest submodule of $M$ whose composition factors lie in $I$, and the \emph{$I$-residual} of $M$ is the smallest submodule such that every composition factor of the quotient lies in $I$. Write $I'$ for $\Irr(H)\setminus I$.

One lemma that we occasionally use, that can be quite powerful, relates the minimal and adjoint modules for exceptional groups. We place it here because there seems no more appropriate place.

\begin{lemma}\label{lem:relatingvminlg} Let $\bG$ be one of $F_4$, $E_6$ and $E_7$.
\begin{enumerate}
\item\label{lemi:vmina} Let $\bG=F_4$. If $p=3$ then $L(F_4)$ is a submodule of $\Lambda^2(M(F_4))$. If $p\geq 5$ then $L(F_4)$ is a summand of $\Lambda^2(M(F_4))$.
\item\label{lemi:vminb} Let $\bG=E_6$. If $p=2$ then $L(E_6)$ is a submodule of $M(E_6)\otimes M(E_6)^*$. If $p=3$ then the socle of 
$M(E_6)\otimes M(E_6)^*$ is $1$-dimensional, and quotienting out by this, $L(E_6)^\circ$ is a submodule. If $p\geq 5$ then $L(E_6)$ is a summand of $M(E_6)\otimes M(E_6)^*$.
\item\label{lemi:vminc} Let $\bG=E_7$. If $p=2$ then the socle of 
$\Lambda^2(M(E_7))$ is $1$-dimensional, and quotienting out by this, $L(E_7)^\circ$ is a submodule. If $p=3$ then $L(E_7)$ is a submodule of $S^2(M(E_7))$. If $p\geq 5$ then $L(E_7)$ is a summand of $S^2(M(E_7))$.
\end{enumerate}
\end{lemma}
\begin{proof} In characteristic $0$, the highest weight modules in $\Lambda^2(M(F_4))$ are $L(\lambda_1)=L(F_4)$ and $L(\lambda_3)$, of dimension $273$. If $p\geq 5$ these two modules remain irreducible, so the exterior square is the sum of these, but $L(\lambda_3)$ has dimension $196$ when $p=3$, so that the exterior square of $M(F_4)$ -- which has dimension $300$ as $M(F_4)$ has dimension $25$ -- has three composition factors: two copies of $L(\lambda_1)$ and one of $L(\lambda_3)$. As the exterior square is self-dual, either this module has the form $52/196/52$ or there is a $52$- or $196$-dimensional summand. However, the regular unipotent element of $F_4$ acts on $M(F_4)$ with blocks $15,9,1$ (see Table \ref{t:unipotentF4}) and thus on the exterior square with blocks $27,21^2,18^6,15^2,9^{10},3$, all of which are divisible by $3$, so there is no simple summand of the exterior square. This proves (\ref{lemi:vmina}).

For characteristic $0$, $M(E_6)\otimes M(E_6)^*=L(\lambda_1)\otimes L(\lambda_6)$ has composition factors the highest weight modules $L(0)$, $L(\lambda_2)=L(E_6)$ and $L(\lambda_1+\lambda_6)$ (of dimension $650$). These again remain irreducible for $p\geq 5$, so we obtain the result. In characteristic $2$, $L(\lambda_1+\lambda_6)$ has dimension $572$ and a copy of $L(\lambda_2)$ is the other composition factor of the Weyl module $W(\lambda_1+\lambda_6)$. Thus we get $L(0)\oplus (L(\lambda_2)/L(\lambda_1+\lambda_6)/L(\lambda_2))$: the trivial breaks off as a summand as the module is self-dual and has a trivial submodule, and the easiest way to check that the second summand is indecomposable is to prove it for $E_6(2)$ with a computer, where we indeed obtain 
\[1\oplus (78/572/78).\]
In characteristic $3$, the composition factors become $L(0)^3,L(\lambda_2)^2,L(\lambda_1+\lambda_6)$. Again, the easiest way to deduce the structure is to test it for $E_6(3)$ using a computer, and note that it has form
\[ 1/77/1,572/77/1,\]
hence must for any group of type $E_6$ because it must be a refinement of this structure and remain self-dual.

For $E_7$, in characteristic $0$, $S^2(M(E_7))$ has composition factors the highest weight modules $L(\lambda_1)=L(E_7)$ and $L(2\lambda_7)$ of dimension $1463$. These both remain irreducible for $p\geq 5$, and so $S^2(M(E_7))$ is the sum of these. For $p=3$, $L(2\lambda_7)$ has dimension $1330$, and the structure is $L(\lambda_1)/L(2\lambda_7)/L(\lambda_1)$. Again, this is most easily checked with a computer for $E_7(3)$. For $p=2$ we take the exterior square, which has composition factors of dimension $1,1,132,132,1274$, and as with $E_6$, the easiest way to check the structure is with a computer for $E_7(2)$, where we get
\[ L(0)/L(\lambda_1)/L(\lambda_6)/L(\lambda_1)/L(0).\]
This completes the proof.
\end{proof}

In many cases we want to prove that a module has a particular composition factor as a submodule or quotient, often the trivial module, which we denote by $k$ or $1$. Thus we need a method of proving that a particular composition factor is always a submodule or quotient in any module with those factors. This is the idea of pressure.

Suppose that $H$ is a finite group such that $O^p(H)=H$, and such that for all simple modules $M$ over a field $k$, $H^1(H,M)=H^1(H,M^*)$. The \emph{pressure} of a module $V$ for $H$ is the quantity
\[ \sum_{M\in\cf(V)} (\dim H^1(H,M)-\delta_{M,k}),\]
where $\delta$ is the Kronecker delta. Results on pressure have occurred in the literature before, with the most general so-far being \cite[Lemma 1.8]{craven2015un2}. Another generalization of this allows us to understand the situation of forcing a module from a collection $\mathcal M$ of simple modules to be a submodule of a given module $V$. If $\mathcal M$ is a collection of simple modules for a group $H$, with $\Ext^1(M,M')=0$ for all $M,M'\in\mathcal M$, and such that $\Ext^1(A,M)=\Ext^1(M,A)$ for all simple modules $A$ and $M$ with $M\in\mathcal M$, then the \emph{$\mathcal M$-pressure} of a module $V$ is the quantity
\[ \sum_{M'\in \cf(V)}\sum_{M\in \mathcal M}(\dim\Ext^1(M,M')-\delta_{M,M'}).\]
The result \cite[Lemma 1.8]{craven2015un2} directly generalizes to $\mathcal M$-pressure, with the exact same proof, so we simply state the result.

\begin{lemma}\label{lem:pressure} Suppose that $H$ is a finite group, and let $\mathcal M$ be a set of simple modules for $H$ such that $\Ext^1(M,M')=0$ for all $M,M'\in \mathcal M$, and $\Ext^1(M,A)=\Ext^1(A,M)$ for all $M\in \mathcal M$ and all simple modules $A$. Let $V$ be a module for $H$ of $\mathcal M$-pressure $n$.
\begin{enumerate}
\item If $n<0$ then $\Hom(M,V)\neq 0$ for some $M\in \mathcal M$, i.e., $V$ has a simple submodule isomorphic to some $M\in\mathcal M$. If $n=0$ then either $\Hom(M,V)\neq 0$ or $\Hom(V,M)\neq 0$, i.e., $V$ has either a simple submodule or quotient isomorphic to some member of $\mathcal M$.

\item More generally, if a composition factor of $V$ has $\mathcal M$-pressure greater than $n$, then either $\Hom(M,V)\neq 0$ or $\Hom(V,M)\neq 0$ for some $M\in\mathcal M$.

\item If $\Hom(M,V)=\Hom(V,M)=0$ for all $M\in\mathcal M$, then any subquotient $W$ of $V$ has $\mathcal M$-pressure between $-n$ and $n$.
\end{enumerate}
\end{lemma}

The concept of pressure can be used to prove that either $M(\bG)$ or $L(\bG)$ possesses a trivial submodule or quotient when restricted to $H$. We therefore would like to know whether that is enough in some circumstances to conclude that $H$ is contained within a positive-dimensional subgroup of $\bG$. The next result is \cite[Lemma 1.4]{craven2015un2}.

\begin{lemma}\label{lem:smallsubspaces} Let $\bG$ be one of $F_4$, $E_6$, ${}^2\!E_6$, $E_7$ or $E_8$. Let $H\leq \bG$. If one of the following holds, then $H$ is contained in a positive-dimensional subgroup of $\bG$:
\begin{enumerate}
\item $H$ stabilizes a $1$-space or hyperplane of $M(\bG)$ or $L(\bG)$;
\item $\bG=F_4$, $E_6$, ${}^2\!E_6$ or $E_7$, and $H$ stabilizes a $2$-space or a space of codimension $2$ in $M(\bG)$;
\item $\bG=E_6$ or ${}^2\!E_6$, and $H$ stabilizes a $3$-space or a $24$-space of $M(E_6)$.
\end{enumerate}
\end{lemma}

In Propositions \ref{prop:fixlineonLG}, \ref{prop:fixlineonMG} and \ref{prop:fix2spaceonMG}, we extend the statements about stabilizing a line of $L(\bG)^\circ$ or $M(\bG)$, or a $2$-space of $M(\bG)$, to include stability under outer automorphisms of the finite group $G$. This allows such statements to be used to deduce the results in the introduction about maximal subgroups.

We end with giving the line stabilizers for the minimal modules for the finite groups $E_6(q)$ and $E_7(q)$. These have appeared in the literature before, and we take these from \cite[Lemmas 5.4 and 4.3]{liebecksaxl1987}.

\begin{lemma}\label{lem:e6stabs} Let $G=E_6(q)$. There are three orbits of lines of the action of $G$ on $M(E_6)$, with line stabilizers as follows:
\begin{enumerate}
\item $F_4(q)$ acting on $M(E_6)$ as $L(\lambda_4)\oplus L(0)$ ($L(0)/L(\lambda_4)/L(0)$ in characteristic $3$);
\item a $D_5$-parabolic subgroup; $q^{16}D_5(q).(q-1)$, acting uniserially as \[L(\lambda_1)/L(\lambda_4)/L(0);\]
\item a subgroup $q^{16}.B_4(q).(q-1)$ acting indecomposably as \[L(0)/L(\lambda_4)/L(0),L(\lambda_1).\]
\end{enumerate}
\end{lemma}


\begin{lemma}\label{lem:e7stabs} Let $G=E_7(q)$. There are five orbits of lines of the action of $G$ on $M(E_7)$, with line stabilizers as follows:
\begin{enumerate}
\item $E_6(q).2$ (the graph automorphism) acting semisimply with composition factors of dimensions $54,1,1$;
\item ${}^2\!E_6(q).2$ (the graph automorphism) acting semisimply with composition factors of dimensions $54,1,1$;
\item an $E_6$-parabolic subgroup $q^{27}.E_6(q).(q-1)$ acting uniserially as \[L(0)/L(\lambda_1)/L(\lambda_6)/L(0);\]
\item a subgroup $q^{1+32}.B_5(q).(q-1)$ acting indecomposably as \[L(0),L(\lambda_1)/L(\lambda_5)/L(0),L(\lambda_1);\]
\item a subgroup $q^{26}.F_4(q).(q-1)$ acting indecomposably as \[L(0),L(0)/L(\lambda_4)/L(\lambda_4)/L(0),L(0).\]
\end{enumerate}
\end{lemma}


\endinput


==> 4maxsubspaces.tex <==
\chapter{Maximal Subgroups and Subspace Stabilizers}
\label{ch:maxsubspace}

The purpose of this chapter is to prove some sufficiency criteria for a subgroup to be strongly imprimitive, essentially making upgrading `Lie imprimitive' to `strongly imprimitive' a formal process in many cases.

Lemma \ref{lem:smallsubspaces} stated that if a subgroup $H$ stabilizes a line or hyperplane on $M(\bG)$ or $L(\bG)^\circ$ then $H$ is Lie imprimitive. Propositions \ref{prop:fixlineonLG} and \ref{prop:fixlineonMG} generalize this to show that $H$ is strongly imprimitive, but we have to place some technical conditions on $H$ that are always satisfied if $H$ is a simple group that is a candidate to be an almost simple maximal subgroup. We also show the same result if $H$ stabilizes a $2$-space on $M(\bG)$ in Proposition \ref{prop:fix2spaceonMG}. If a subgroup $H$ is a blueprint for a special class of module, usually including $M(\bG)$ or $L(\bG)^\circ$, then we again can use this to prove strong imprimitivity, see Proposition \ref{prop:blueprintissi}. The general criterion is Proposition \ref{prop:intersectionstabilizers}, which is reproduced from \cite[Section 4.2]{litterickmemoir}, itself generalizing work of \cite[Proposition 1.12]{liebeckseitz1998}.

These results will be used in Chapters \ref{ch:f4} to \ref{ch:e7oddsl} to prove strong imprimitivity given information about subgroups $H$ of $\bG$.

\medskip

We recall some definitions: a subgroup $H$ of $\bG$ is \emph{$\bG$-completely reducible} if, whenever $H$ is contained in a parabolic subgroup of $\bG$, it is contained in the corresponding Levi subgroup; it is \emph{$\bG$-irreducible} if $H$ is not contained in any parabolic subgroup of $\bG$; as we have seen before, it is \emph{Lie primitive} if it is not contained in any proper positive-dimensional subgroup of $\bG$.

The first result that we need is by Liebeck, Martin and Shalev \cite[Proposition 2.2 and Remark 2.4]{liebeckmartinshalev2005}, and this is translated into our notation.

\begin{proposition}\label{prop:paraisgood} Let $H$ be a finite subgroup of $\bG$ such that $H$ is not $\bG$-completely reducible and $H\leq \bG^\sigma$. There exists a proper parabolic subgroup $\bP$ of the $\bG$ such that $H$ is contained in $\bP$ and $\bP$ is both $\sigma$-stable and $N_{\Aut^+(\bG)}(H)$-stable. In particular, $H$ is strongly imprimitive.
\end{proposition}

If $R$ is an elementary abelian $r$-group such that $N_{\bG}(R)$ is an exotic $r$-local subgroup then of course $R$ is contained in the normalizer of a torus but $N_{\bG}(R)$ is Lie imprimitive, so that $R$ is Lie imprimitive but not strongly imprimitive. Thus one cannot prove that every Lie imprimitive subgroup is strongly imprimitive. If one takes the non-toral $3^3$ in $F_4(\mathbb{C})$ (which was constructed in \cite{griess1991}, for example), then its normalizer $3^3\rtimes \SL_3(3)$ is an exotic $3$-local subgroup, and the subgroup $3^3$ stabilizes a $2$-space on $M(F_4)$. (The easiest way to see this is to note that the $3^3$ is the Sylow $3$-subgroup of the Lie primitive $\PSL_2(27)$, which acts irreducibly on $M(F_4)$ (see \cite{cohenwales1997} or \cite{liebeckseitz2004a} for example), and each $26$-dimensional module for $\PSL_2(27)$ restricts to its Sylow $3$-subgroup with composition factors of dimension $2$.)

Thus one will not be able to prove a general statement that if $H$ is a finite subgroup of $F_4$ and stabilizes a $2$-space on $M(F_4)$ then $H$ is strongly imprimitive, since it is not true. We therefore place some restrictions on $H$. We are looking for subgroups $H\leq \bG^\sigma$ such that $N_{\bG^\sigma}(H)$ is almost simple modulo the centre of $\bG^\sigma$, so in particular $C_{\bG^\sigma}(H)=Z(\bG^\sigma)$. This latter condition is enough.

\begin{proposition}\label{prop:Gcrisgood} Suppose that $H$ is a finite subgroup of $G=\bG^\sigma$ such that $C_G(H)=Z(G)$. If $H$ is $\bG$-reducible then $H$ is strongly imprimitive.
\end{proposition}
\begin{proof} Suppose that $H$ is not strongly imprimitive, and that $H$ is $\bG$-reducible. By Proposition \ref{prop:paraisgood}, $H$ is $\bG$-completely reducible, so $H$ is contained in a proper ($\sigma$-stable) Levi subgroup $\bL$. Since $C_{\bG}(\bL)$ contains a torus $\bT$ of $\bG$, $\bY=C_{\bG}(H)^\circ\neq 1$. Note that $\bY$ is $\sigma$-stable and $N_{\Aut^+(\bG)}(H)$-stable, since $H$ is, and the same holds for $C_{\bG}(\bY)$. This latter subgroup contains $H$, so if it is infinite then $H$ is strongly imprimitive.

If $\bY$ is abelian then $\bY\leq C_{\bG}(\bY)$, so we may assume that $\bY$ is not a torus. However, then $\bY^\sigma\neq 1$ (if $\bY^\sigma=1$ then $\bY$ is a torus and $p=2$), and hence $C_G(H)\neq 1$. Since $C_G(H)=1$ by assumption, $\bY$ is a torus, and therefore $H$ is strongly imprimitive, as needed.
\end{proof}

Thus if $H$ is a subgroup of $\bG^\sigma$ such that $N_{\bar G}(H)$ is almost simple, $H$ is $\bG$-irreducible.

The next result comes entirely from \cite[Chapter 4]{litterickmemoir}, particularly \cite[Corollary 4.5]{litterickmemoir}, and is a direct generalization of the methods of \cite[Proposition 1.12]{liebeckseitz1998}. If $W$ is a subspace of a $\bG$-module $V$, write $\bG_W$ for the stabilizer of $W$ in $\bG$, and if $\mathcal W$ is a collection of subspaces of $V$, write $\bG_{\mathcal W}$ for the intersection of the $\bG_W$ for $W\in \mathcal W$. Note that this also applies for $\bG=F_4$ and $p=2$, where the `graph morphism' interchanges $\lambda_i$ and $\lambda_{5-i}$. 

\begin{proposition}\label{prop:intersectionstabilizers} Let $\bG$ be a simple algebraic group over an algebraically closed field, and let $V$ be a semisimple module such that the highest weights of the composition factors are stable under graph morphisms of $\bG$. Let $H$ be a finite subgroup of $\bG$.

If $\phi\in N_{\Aut^+(\bG)}(H)$ then $\phi$ permutes the $H$-invariant subspaces of $V$. Hence if $\mathcal W$ is an orbit of $H$-invariant subspaces of $V$, then $H\leq \bG_{\mathcal W}$ and $\bG_{\mathcal W}$ is $\phi$-stable.

If $\mathcal W$ is one of
\begin{enumerate}
\item all $H$-invariant subspaces of $V$,
\item all $H$-invariant subspaces of $V$ whose dimension lies in some subset $I\subseteq \N$,
\item all simple $H$-invariant subspaces of $V$,
\item all simple $H$-invariant subspaces of $V$ whose dimension lies in some subset $I\subseteq \N$,
\end{enumerate}
then $\mathcal W$ is a union of orbits of $H$-invariant subspaces of $V$. In particular, $\bG_{\mathcal W}$ is a subgroup of $\bG$ containing $H$ and stable under every element of $N_{\Aut^+(\bG)}(H)$.

Hence if $\bG_{\mathcal W}$ is positive dimensional for one of these sets $\mathcal W$ of subspaces, not stabilized by $\bG$ itself, then $H$ is strongly imprimitive.
\end{proposition}

This also gives us the following result, applying the statement to blueprints.

\begin{proposition}
\label{prop:blueprintissi} Suppose that $H$ is a finite subgroup of $\bG$, and let $V$ be a semisimple module that is $N_{\Aut^+(\bG)}(H)$-stable, i.e., $V$ is a sum of highest-weight modules whose weights form orbits under the action of the graph morphisms in $N_{\Aut^+(\bG)}(H)$. If $H$ is a blueprint for $V$, then either $H$ is strongly imprimitive or $H$ acts irreducibly on every composition factor of $V$.

In particular, if $H$ is either $\PSL_2(p^a)$ or $\SL_2(p^a)$ in $\bG=E_7$ with $Z(H)=Z(\bG)$, and $H$ is a blueprint on either $M(\bG)$ or $L(\bG)^\circ$, then $H$ is strongly imprimitive.
\end{proposition}
\begin{proof} The first part is a direct consequence of Proposition \ref{prop:intersectionstabilizers}. The second statement follows from the first if $H$ cannot act irreducibly on either $M(\bG)$ or $L(\bG)^\circ$. But this follows from \cite{liebeckseitz2004a}.
\end{proof}

We now prove results about stabilizing lines on $L(\bG)$ and $M(\bG)$, and $2$-spaces on $M(\bG)$.

\begin{proposition}\label{prop:fixlineonLG} If $H$ is a finite subgroup of $G=\bG^\sigma$ such that $C_G(H)=Z(G)$, and $H$ stabilizes a line on $L(\bG)^\circ$, then $H$ is strongly imprimitive.
\end{proposition}
\begin{proof} Suppose that the fixed-point subspace of $H$ on $L(\bG)$ is $W\neq 0$, and we consider $\bG$ to be of adjoint type, so that $L(\bG)$ cannot have a trivial submodule \cite[Lemma 2.1.1]{liebeckseitz2004}. By \cite[(1.3)]{seitz1991}, if $W$ contains a nilpotent element then $H$ is contained in a proper parabolic subgroup, hence by Proposition \ref{prop:Gcrisgood} $H$ is strongly imprimitive.

Thus $W$ consists of semisimple elements. Indeed, since $W$ is the space of fixed points of $H$ on $L(\bG)$, it is a subalgebra of $L(\bG)$. This means that $W$ is contained in a maximal torus of $L(\bG)$, hence (as in \cite[(1.3)]{seitz1991}) $\bC=C_{\bG}(W)$ contains a maximal torus of $G$. Since $H\leq \bC$, this means that $\bC$ is a maximal-rank subgroup of $\bG$, and is $\sigma$-stable since $W$ is. To show invariance under $N_{\bar G}(H)$, we now apply Proposition \ref{prop:intersectionstabilizers}, since $\bC$ is the intersection of the stabilizers of all $H$-invariant $1$-spaces of $L(\bG)$. This shows that $\bC$ is $N_{\Aut^+(\bG)}(H)$-stable, so $H$ is strongly imprimitive.
\end{proof}

We now do the same thing with $M(\bG)$ in place of $L(\bG)$. We add a small condition on $H$ that is certainly satisfied for simple groups. This can probably be removed, at the expense of making the proof more complicated.

\begin{proposition}\label{prop:fixlineonMG} If $H$ is a finite subgroup of $G=\bG^\sigma$ such that $C_G(H)=Z(G)$, $H$ has no subgroup of index $2$, and $H$ stabilizes a line on $M(\bG)$, then $H$ is strongly imprimitive.
\end{proposition}
\begin{proof} Suppose that the fixed-point subspace $M(\bG)^H$ of $H$ on $M(\bG)$ is non-zero. If $\bG=F_4$ and $p=2$ then as $M(F_4)$ is a submodule of $L(F_4)$, we get the result in this case by Proposition \ref{prop:fixlineonLG}. If $p$ is odd, then $H$ is contained in a line stabilizer of $M(F_4)$, which from \cite[Lemma 2.2(iii)]{liebeckseitz2005} are contained in either a maximal parabolic or $B_4$. In the first case, we apply Proposition \ref{prop:Gcrisgood} to obtain the result, so $H$ is contained in $B_4$.

If $M(\bG)^H$ has dimension $1$ or $2$ then the centralizer of $M(\bG)^H$ is positive dimensional, and hence we may apply Proposition \ref{prop:intersectionstabilizers} to obtain the result, as in the previous proposition. Thus $M(\bG)^H$ has dimension at least $3$, and so centralizes a $2$-space on the sum of the natural and spin modules for $B_4$. Note that $H$ cannot lie in a parabolic subgroup of $B_4$ since it does not lie in a parabolic subgroup of $F_4$, and hence $H$ cannot lie in a $B_3$ subgroup of $B_4$, which is the $2$-space centralizer on the natural module. On the other hand, since the spin module for $B_4$ appears in both $M(F_4)$ and $L(F_4)$, if $H$ stabilizes a line on the spin module then $H$ stabilizes a line on $L(F_4)$, and we apply Proposition \ref{prop:fixlineonLG}.

If $G=E_6$ then from Lemma \ref{lem:e6stabs} the line stabilizers are $F_4$ or subgroups contained in parabolic subgroups, so $H\leq F_4$. If $H$ stabilizes a point on $M(F_4)$ then we apply the previous paragraph, and if $H$ does not then $H$ stabilizes a unique line on $M(E_6)$, whence we apply Proposition \ref{prop:intersectionstabilizers} again.

If $G=E_7$ then from Lemma \ref{lem:e7stabs}, we may assume that $H$ only stabilizes lines whose stabilizers are of the form $E_6.2$, as all others are contained in maximal parabolic subgroups and we again apply Proposition \ref{prop:Gcrisgood}. However, since $H$ has no subgroup of index $2$, this means that $H$ is contained in an $E_6$-Levi subgroup, and again we apply Proposition \ref{prop:Gcrisgood}. This completes the proof.
\end{proof}

We also will have cause to use $2$-space stabilizers on $M(\bG)$ for $\bG=F_4,E_6,E_7$. By dimension counting (see Lemma \ref{lem:smallsubspaces}) we see that the stabilizer of such a space is positive dimensional so $H$ is imprimitive, but we need to show that $H$ is strongly imprimitive. Because the proof of this goes case by case, we only prove the precise cases that we need, rather than produce a general method. Even with this restriction, the proof is long and technical.

\begin{proposition}\label{prop:fix2spaceonMG} If $H=\SL_2(p^a)$ is a subgroup of $\bG$ for $\bG=F_4,E_6,E_7$ and $p=2$, or $\bG=E_7$ and $p^a=5,7,9,25,27,49$, and $H$ stabilizes a $2$-space on $M(\bG)$, then $H$ is strongly imprimitive.
\end{proposition}
\begin{proof} If $p$ is odd then any group that normalizes $H$ centralizes $Z(H)$, so either lies in the centralizer of an involution -- hence $H$ is strongly imprimitive -- of $Z(H)=Z(\bG)$. Thus for $p$ odd we assume that $Z(H)=Z(\bG)$. In addition, if $H$ is $\bG$-reducible then $H$ is strongly imprimitive by Proposition \ref{prop:Gcrisgood}, so we may assume that $H$ is $\bG$-irreducible. By Lemma \ref{lem:smallsubspaces}, $H$ is not Lie primitive.

Let $\bX$ be a minimal $\bG$-irreducible subgroup of $\bG$ containing $H$, so that $H$ is Lie primitive in $\bX$. If $\bX$ is a product of groups then the projections along each must also be Lie primitive, else we could replace $\bX$ with a smaller subgroup. There are no Lie primitive subgroups $\SL_2(p^a)$ in classical groups or $G_2$ by Proposition \ref{prop:morphismextensiontrueforclassical}, so if $\bX$ has a classical or $G_2$ component then this is $A_1$. Thus $\bX$ can only have components $A_1$, $F_4$ and $E_6$. Furthermore, since there are no Lie primitive copies of $H$ in a product of $A_1$s, there is at most one $A_1$ component in $\bX$. Note that, of course, $\bX$ is not necessarily $\sigma$-stable, never mind $N_{\Aut^+(\bG)}(H)$-stable.

\medskip

If $\bG=F_4$ (and hence $p=2$) then $\bX$ is an $A_1$ subgroup. If $\bX\leq B_4$ then $\bX$ and hence $H$ stabilizes a line on $M(F_4)$, whence $H$ is strongly imprimitive by Proposition \ref{prop:fixlineonMG}. However, $\bX\leq B_4$ by \cite[Table 5]{thomas2016}, completing the proof for $F_4$.

\medskip

If $\bG=E_6$ (and again $p=2$), then instead of this analysis, which would also work, we use the tables of Cohen--Cooperstein \cite{cohencooperstein1988} to determine the possibilities for the $2$-space $W$ being stabilized, and see that in all cases $C_{\bG}(W)$ must have a unipotent radical, hence $H$ lies in a parabolic, hence is strongly imprimitive by Proposition \ref{prop:Gcrisgood}.

\medskip

For $\bG=E_7$ and all primes $p$, then as $\bX\neq \bG$, either $\bX=A_1$, or it involves $F_4$ or $E_6$. If $\bX$ involves $E_6$ then $\bX=E_6$ is a Levi subgroup, and if $\bX=F_4$ then $\bX\leq E_6$, so again $H$ is not $\bG$-irreducible. Thus $\bX$ is either $F_4A_1$ or $A_1$. 

If $\bX=F_4A_1$ then the projection of $H$ along $F_4$ must be Lie primitive in $F_4$, else $\bX$ is contained in a proper positive-dimensional subgroup of $F_4A_1$, and these are all classical, so $\bX=A_1$. In this case, the best way to proceed is to use Theorem \ref{thm:f4}, which we prove in Chapter \ref{ch:f4}, which states that there are no Lie primitive copies of $\PSL_2(p^a)$ in $F_4$. Using this result is valid and not circular reasoning, since we will not need to use this result for $E_7$ until Chapter \ref{ch:e7oddsl}, by which time Theorem \ref{thm:f4} will have been proved.

Thus for the rest of the proof, $\bX$ is an irreducible $A_1$ subgroup of $E_7$. If $p=2$ then $\bX\leq D_6A_1$ by \cite[Table 7]{thomas2016}, so since $D_6A_1$ stabilizes a line on $L(E_7)^\circ$, $H$ is strongly imprimitive by Proposition \ref{prop:fixlineonLG}. Thus $p$ is odd.

The information given in \cite[Tables 7 and 12]{thomas2016} is significant, but does not include the (non-trivial) unipotent class intersecting $\bX$, and we also need the module action of $H$ on $M(E_7)$ in certain cases.

The conditions on the embeddings of the $A_1$s in \cite{thomas2016} are important, as if those conditions are not satisfied then the subgroup is not $\bG$-irreducible. If $H$ is contained in a diagonal $A_1$ subgroup of a product of $A_1$s, then $H$ is contained in other diagonal $A_1$s, obtained by twisting the representations of the projections along the various $A_1$s. Every one of the diagonal $A_1$s containing $H$ must be $\bG$-irreducible.

The effect of this is, for each class of $A_1$ in the tables, we require that the conditions are satisfied for integers lying between $0$ and $a-1$, else we may replace one, say $i$, by $i-a$, and yield another $A_1$ subgroup containing $H$. The consequence is that $a$ needs to be large enough so that the conditions can still hold.

For example, if $p=3$ then from \cite[Table 7]{thomas2016} we see that $A_1$ subgroups with labels $3$, $10$, $11$ and $12$ exist. For subgroup $11$, the centre of it does not coincide with the centre of $\bG$, so this can be excluded for all primes. Subgroup $3$ requires $a\geq 3$ for the conditions to be satisfied, subgroup $10$ requires $a\geq 2$, and subgroup $12$ cannot occur for $a\leq 3$.

In what follows, we use the notation for simple modules for $\SL_2$ from Chapter \ref{ch:sl2modules}, because it is much easier to understand the dimensions of the composition factors than using the notation $L(\lambda)$. We will show that the simultaneous stabilizer of all $2$-dimensional submodules of $M(E_7)\downarrow_H$ is positive dimensional, and therefore apply Proposition \ref{prop:intersectionstabilizers}, as we did in Propositions \ref{prop:fixlineonLG} and \ref{prop:fixlineonMG}, to prove that $H$ is strongly imprimitive, completing the proof of the result. Note that if $H$ stabilizes a unique $2$-space on $M(E_7)$ then the stabilizer is positive dimensional by Lemma \ref{lem:smallsubspaces}, so we are done in this case.

\medskip

We first set $p=3$, and so $a=2,3$. The subgroup $\bX$ must be either subgroup $3$ or subgroup $10$ from \cite[Table 7]{thomas2017un}, both lying inside $A_1D_6$. For subgroup $3$ we require $a=3$, and may assume that the action of $H$ along $M(D_6)$ is $L(1)\otimes L(1)^{[1]}\otimes L(2)^{[2]}$ (where $[i]$ denotes $i$ field twists, so $L(1)^{[1]}=L(3)$), and the action along $A_1$ is $L(1)^{[i]}$ for $i=0,1,2$. Thus in the notation of \cite{thomas2016}, $r=0,1,2$, ${u,t}={0,1}$ (both possibilities are allowed), $s=2$, and in our notation from Chapter \ref{ch:sl2modules} the two modules are $12_{1,2,3}$ and $2_i$ for $i=1,2,3$.

Since $\bX$ lies in $A_1D_6$, $\bX$ acts on $M(E_7)$ as the sum of (the restrictions to $\bX$ of) $(M(A_1),M(D_6))$ and $(L(0),L(\lambda_5))$. The three possibilities for the action of $H$ on $(M(A_1),M(D_6))$ are
\[ 6_{2,3}\oplus 18_{2,1,3},\quad 6_{1,3}\oplus 18_{1,2,3},\quad 8/2_2,6_{2,1}/8.\]
The other summand of $M(E_7)\downarrow_H$ does not depend on $i$, but does depend on which of $u$ and $t$ is $0$ and $1$. From \cite[Table 12]{thomas2016} we can read off the factors of $M(E_7)\downarrow_{\bX}$ and hence of $M(E_7)\downarrow_H$. These are
\[ 18_{2,1,3},8,2_2^2,2_3\quad\text{and}\quad 18_{1,2,3},6_{3,1},2_1^2,2_2,2_3\]
according as $t=0$ and $t=1$ respectively. The (non-trivial) unipotent element in $H$ belongs to class $2A_2+A_1$ by \cite[4.10]{lawther2009}, which acts on $M(E_7)$ with Jordan blocks $3^{18},1^2$ by \cite[Table 7]{lawther1995}. In particular, since there are no blocks of size $2$, there are no $2$-dimensional summands of $M(E_7)\downarrow_H$, and since $2_2$ and $2_1$ respectively are the only composition factors to appear more than once, they must lie in the socle and top of $M(E_7)\downarrow_H$. In particular, $H$ stabilizes a unique $2$-space, so we are done.

For subgroup $10$, we can have either $p^a=9$ or $p^a=27$. If $p^a=9$, then the parameters of $\bX$ from \cite{thomas2016} are $s=0$, $t=1$, and $r,u=0,1$, up to field automorphism. The unipotent class of $E_7$ to which a non-trivial unipotent element of $H$ belongs is again $2A_2+A_1$, so again there are no $2$-dimensional summands of $M(E_7)\downarrow_H$. The restriction of $(M(A_1),M(D_6))$ to $H$  is the sum of the modules $2_r\otimes 9$ and $2_{r+1}\otimes 3_{u+1}$. The first of these is the projective cover of a $6$-dimensional module, and the second of these contains a $2$-dimensional submodule if and only if $r=u$, in which case it is of the form $2_{u+1}/2_{u+2}/2_{u+1}$. The restriction of $(L(0),L(\lambda_5))$ to $H$ has the form
\[(4/1,1,3_1,3_2/4)\otimes 2_{u+1}.\]
The submodule $1,1,3_1,3_2/4$ is uniquely defined, and its product with $2_{u+1}$ has a single $2_{u+2}$ in the socle and no $2_{u+1}$. The top of this tensor product is $4\otimes 2_{u+1}=2_{u+2}\oplus 6_{u+2,u+1}$, but the $2_{u+2}$ cannot become a submodule for then it would be a summand, and there are no $2$-dimensional summands. Thus the $2$-dimensional factors of the socle of $M(E_7)\downarrow_H$ are $2_{u+2}$ if $r\neq u$, and $2_{u+1}\oplus 2_{u+2}$ if $r=u$.

In the former case $H$ stabilizes a unique $2$-space on $M(E_7)$ so we are done, so assume the latter holds. Notice that the irreducible $A_1$ subgroup $\bX$ with the parameters above also stabilizes the $2_{u+1}$ and the $2_{u+2}$, so the simultaneous stabilizer of both contains $\bX$ and we are done.

For $p^a=27$, we need $s<t$, and so $s=0$, $t=1$ or $s=0$, $t=2$ up to field automorphism, with $0\leq u,r\leq 2$. Suppose first that $s=0$ and $t=1$; this is very similar to the case for $p^a=9$. The restriction of $(M(A_1),M(D_6))$ to $H$ contains the modules $2_r\otimes 3_s\otimes 3_t$ and $2_r\otimes 3_u$, and the only way to get a $2$-dimensional submodule is if $r=u$, in which case we get the summand $2_{u+1}/2_{u+2}/2_{u+1}$. For the contribution from $(L(0),L(\lambda_5))$, the structure is
\[ (4_{1,2}/1,3_2,4_{1,3}/4_{1,2})\otimes 2_{u+1}.\]
This tensor product has at most one copy of a $2$-dimensional module in the socle, and the subgroup $\bX$ stabilizes each of these potential $2$-dimensional submodules if they exist, and we are done.

If $s=0$ and $t=2$ instead then the same statements for $(M(A_1),M(D_6))$ hold. The structure of $(L(0),L(\lambda_5))$ also very similar, being
\[ (4_{1,3}/1,3_1,4_{2,3}/4_{1,3})\otimes 2_{u+1}.\]
The same statements about $2$-dimensional submodules hold as well, proving the result in this case.

\medskip

We now set $p=5$. For $p^a=5$, we see from \cite[Table 7]{thomas2016} that there are no $\bG$-irreducible subgroups $H$. For $p^a=25$, we can satisfy the conditions for subgroups $8$, $9$, $10$ and $19$ from Thomas's list. The first three lie in $A_1D_6$, the last in $A_1A_1$.

The first case is subgroup $8$: here $s\neq t$ and $u\leq v$. By field automorphism we may assume that $s=0$ and $t=1$, and $u,v=1,2$. The action of $H$ on the module $(M(A_1),M(D_6))$ is
\[ 2_{r+1}\otimes (5_1\oplus 3_2\oplus 2_{u+1}\otimes 2_{v+1}).\]
Any $2$-dimensional submodule of this is stabilized by $\bX$, so we consider the restriction of $(L(0),L(\lambda_5))$ to $\bX$ and $H$. This is
\[ 4_1\otimes 2_2\otimes(2_{u+1}\oplus 2_{v+1}),\]
and this yields $2$-dimensional submodules if $u=1$ or $v=1$, again stabilized by $\bX$ as well. Hence $H$ and $\bX$ stabilize the same $2$-dimensional subspaces of $M(E_7)$, so we are done.

For subgroup $9$, we may take $s=0$, $t=u=1$, and $r=1,2$. The composition factors of the restriction of $(L(0),L(\lambda_5))$ to $H$ are $10_{2,1}^2,6_{2,1}^2$, so we may concentrate on $(M(A_1),M(D_6))$. The action of both $H$ and $\bX$ on this is
\[ 2_{r+1}\otimes (5_1\oplus 3_1\oplus 2_2^{\otimes 2}).\]
Both the $H$-action and $\bX$-action have two $2$-dimensional composition factors in the socle for either $r=1$ or $r=2$, so again the intersection of the stabilizers of all $2$-dimensional submodules of $M(E_7)\downarrow_H$ is positive dimensional.

For subgroup $10$, here we may take $s=0$, $t=1$ and $r,u=1,2$. We have four composition factors of $M(E_7)\downarrow_{\bX}$, and the restrictions to $H$ of these are:
\begin{itemize}
\item $2_{r+1}\otimes 3_1\otimes 3_2$, which is $(2_{r+1}\oplus 4_{r+1})\otimes 3_{r+2}$;
\item $2_{r+1}\otimes 3_{u+1}$, which is $6_{u+1,r+1}$ if $u\neq r$ and $2_{u+1}\oplus 4_{u+1}$ if $u=r$;
\item $4_1\otimes 2_2\otimes 2_{u+1}$ and $4_2\otimes 2_1\otimes 2_{u+1}$, and these two are $(3_{u+1}\oplus 5_{u+1})\otimes 2_{u+2}$ and $(1\oplus 3_{u+1})\otimes 4_{u+2}$.
\end{itemize}
We see that there is a unique $2$-dimensional submodule if $u=r$, and none otherwise, and so we are done.

If the subgroup is $19$, then the action of $\SL_2(5)$ on $M(E_7)$ is
\[P(4)^{\oplus 4}\oplus (2/2,4)\oplus (2,4/2),\]
and one of the $2$-dimensional submodules is distinguishable as being contained in a module $2/2$. Thus either $H$ stabilizes a unique $2$-space, and we are done by Proposition \ref{prop:intersectionstabilizers}, or it stabilizes the same number of subspaces as the copy of $L=\SL_2(5)$ inside it, in which case it stabilizes the subspace that must lie in a singleton orbit, and again we are done.

\medskip

The final case is $p=7$. In this case, we simply consider all subgroups from Thomas's list that occur for $p=7$, and tabulate their restrictions to $H=\SL_2(7)$.
\begin{center}\begin{tabular}{ccc}
\hline Group Number & Unipotent class & Action on $M(E_7)$
\\ \hline $1$, $2$, $6$, $16$, $19$ & $E_7(a_5)$ & $P(6)^{\oplus 2}\oplus P(4)\oplus 6\oplus 4^{\oplus 2}$
\\ $3$, $8$, $9$, $10$ & $A_3+A_2+A_1$ & $6^{\oplus 3}\oplus 4^{\oplus 7}\oplus 2^{\oplus 5}$
\\ $7$ & $D_5(a_1)+A_1$ & $P(6)^{\oplus 3}\oplus 4\oplus 2^{\oplus 5}$
\\ $12$ & $A_2+3A_1$ & $4^{\oplus 7}\oplus 2^{\oplus 14}$
\\ $15$, $17$ & $A_6$ & $P(6)\oplus P(4)^{\oplus 2}\oplus P(2)$
\\ \hline
\end{tabular}\end{center}
We exclude those with class $E_7(a_5)$ as $H$ does not stabilize a $2$-space in this case. If the unipotent elements of $H$ come from class $A_6$ then $H$ stabilizes a unique $2$-space on $M(E_7)$, and we are done. From \cite[Table 7]{thomas2016} we see that subgroup 7 is $\bG$-reducible unless $a\geq 3$, so this case cannot occur. The remaining two unipotent classes, $A_3+A_2+A_1$ and $A_2+3A_1$, are generic for $M(E_7)$ in the sense of Definition \ref{defn:genericunipotent} below. Lemma \ref{lem:genericunipotent} states that subgroups containing generic unipotent elements for $M(E_7)$ are strongly imprimitive, and this completes the proof of the result.
\end{proof}


\endinput


==> 6unipotent.tex <==
\chapter{Unipotent and Semisimple Elements}
\label{ch:unipssemis}

This chapter collects together a variety of facts about unipotent and semisimple elements in groups of Lie type. We consider criteria for unipotent and semisimple elements to be blueprints. We then move on to considering modules for $\SL_2$, and how the weight spaces of the module and the eigenvalues of elements of $\SL_2$ interact, with the aim of finding blueprint elements and blueprint subgroups $\PSL_2(p^b)$.

\section{Actions of Unipotent Elements}

Let $\bG$ be a simple algebraic group in characteristic $p$. The Bala--Carter--Pommerening labelling system for the unipotent classes, as used in a slightly modified form (to deal with interpolation of extra classes in certain bad characteristics) in our main reference \cite{lawther1995} for unipotent classes of exceptional groups, gives us a way to discuss unipotent classes that is independent of the characteristic $p$ of $\bG$. We may therefore compare the action of a unipotent class on a fixed simple module for different primes.

As is well known, any matrix of order a power of a prime $p$ defined over a field of characteristic $p$ can be written in Jordan normal form, with the conjugacy class in the general linear group being determined by the sizes of the Jordan blocks. Thus, if $u$ is a unipotent element of $\bG$ then for every module for $\bG$ of dimension $n$ we can associate a partition of $n$, the sizes of the various Jordan blocks in the action of $u$ on the module. We use the notation for this, and unipotent classes, from \cite{lawther1995}, which determines the Jordan block structure of the action of all unipotent classes of exceptional groups on the minimal and adjoint modules.

The only cases we will need that are not covered in \cite{lawther1995} are when $L(\bG)\neq L(\bG)^\circ$ and $M(F_4)$ for $p=3$. The next lemma gives the actions of the unipotent classes on the $25$-dimensional simple module $M(F_4)$, on the $26$-dimensional Weyl module $25/1$, and on the $27$-dimensional minimal module $M(E_6)$ for $E_6$, which has structure $1/25/1$ when restricted to $F_4$.

\begin{lemma}\label{lem:unipotentF4}
Let $u$ be a unipotent element in $F_4(3^n)$. The Jordan blocks of the action of $u$ on the $25$-dimensional minimal module $M(F_4)$, together with the extension $25/1$ and the minimal module $M(E_6)$ for $E_6$ is one of those given in Table \ref{t:unipotentF4}.
\begin{table}
\begin{center}
\begin{tabular}{lccc}
\hline Class in $F_4$ & Action on $M(F_4)$ & Action on $25/1$ & Action on $M(E_6)=1/25/1$
\\\hline $A_1$ & $2^6,1^{13}$ & $2^6,1^{14}$ & $2^6,1^{15}$
\\ $\tilde A_1$ & $3,2^8,1^6$ & $3,2^8,1^7$ & $3,2^8,1^8$
\\ $A_1+\tilde A_1$ & $3^3,2^6,1^4$ & $3^3,2^6,1^5$ & $3^3,2^6,1^6$
\\ $A_2$ & $3^6,1^7$ & $3^6,1^8$ & $3^6,1^9$
\\ $A_2+\tilde A_1$ & $3^7,2^2$ & $3^7,2^2,1$ & $3^7,2^2,1^2$
\\ $\tilde A_2$, $\tilde A_2+A_1$ & $3^8,1$ & $3^8,2$ & $3^9$
\\ \hline $B_2$ & $5,4^4,1^4$ & $5,4^4,1^5$ & $5,4^4,1^6$
\\ $C_3(a_1)$ & $5^2,4^2,3,2^2$ & $5^2,4^2,3,2^2,1$ & $5^2,4^2,3,2^2,1^2$
\\ $F_4(a_3)$ & $5^3,3^3,1$ & $5^3,3^3,1^2$ & $5^3,3^3,1^3$
\\ $B_3$ & $7^3,1^4$ & $7^3,1^5$ & $7^3,1^6$
\\ $C_3$, $F_4(a_2)$ & $9,6^2,3,1$ & $9,6^2,3,2$ & $9,6^2,3^2$
\\ $F_4(a_1)$ & $9^2,7$ & $9^2,7,1$ & $9^2,7,1^2$
\\ \hline $F_4$ & $15,9,1$ & $15,9,2$ & $15,9,3$
\\ \hline
\end{tabular}
\end{center}
\label{t:unipotentF4}\caption{Actions of unipotent elements on $M(F_4)$ and its extensions for $F_4$ in characteristic $3$}
\end{table}
\end{lemma}
\begin{proof}
The Jordan blocks of the actions of the unipotent elements on the $26$-dimensional module are given in \cite[Table 3]{lawther1995}, and using a computer, a representative of each of the classes was constructed in $F_4(3)$. The Jordan blocks of their actions on the $25$-dimensional composition factor were then computed, and are as above. The classes on the $25/1$ are exactly those in \cite[Table 3]{lawther1995}, and the corresponding classes for $E_6$ are in \cite[Table 5]{lawther1995}.
\end{proof}

Using a computer and constructing classes manually is the method by which we prove the next two lemmas, which we include for completeness.

\begin{lemma}\label{lem:unipotentE6}
Let $u$ be a unipotent element in $E_6(3^n)$. The Jordan blocks of the action of $u$ on the $77$-dimensional Lie algebra module $L(E_6)^\circ$ are obtained from the action on $L(E_6)$ by removing a Jordan block of size 1, except in the cases listed in Table \ref{t:unipotentE6}.
\begin{table}
\begin{center}
\begin{tabular}{lcc}
\hline Class in $E_6$ & Action on $L(E_6)^\circ$ & Action on $L(E_6)$
\\\hline $2A_2$&$3^{23},1^8$&$3^{23},2,1^7$
\\$2A_2+A_1$&$3^{24},2^2,1$&$3^{24},2^3$
\\$A_5$&$9^3,8^2,6^4,3^2,1^4$&$9^3,8^2,6^4,3^2,2,1^3$
\\$E_6(a_3)$&$9^4,7,6^4,3^3,1$&$9^4,7,6^4,3^3,2$
\\$E_6(a_1)$&$9^8,5$&$9^8,6$
\\$E_6$&$19,15^2,9^3,1$&$19,15^2,9^3,2$
\\\hline
\end{tabular}
\end{center}
\label{t:unipotentE6}\caption{Actions of unipotent elements on $L(E_6)^\circ$ and $L(E_6)$ for $E_6$ in characteristic $3$, where one does not obtain the former from the latter by removing a trivial Jordan block}
\end{table}
\end{lemma}

\begin{lemma}\label{lem:unipotentE7} Let $u$ be a unipotent element in $E_7(2^n)$. The Jordan blocks of the action of $u$ on the $132$-dimensional Lie algebra module $L(E_7)^\circ$ are obtained from the action on $L(E_7)$ by removing a Jordan block of size 1, for every unipotent class.
\end{lemma}

We can see from the tables in \cite{lawther1995} that for every unipotent class there is a set of primes $P$ such that, for any prime $p\not\in P$ the partition describing the Jordan block structure on a fixed module $V$ is the same.

\begin{definition}\label{defn:genericunipotent} Let $\bG$ be an algebraic group and let $V$ be a highest weight module for $\bG$. Let $u$ be a unipotent element of $\bG$. If the Jordan block structure of $u$ on $V$ is the same as for cofinitely many primes, then $u$ is said to be \emph{generic} on $V$.
\end{definition}

Thus, informally, the non-generic classes are those where the prime is in the set $P$ described above, where the partition differs from the `usual' one.

The reason that generic unipotent classes are interesting is that we can find `nice' $A_1$ subgroups containing them, at least if the class has elements of order $p$. In \cite[Lemma 1.2]{craven2015un2} we show that such unipotent elements are blueprints for $M(\bG)$ and, indeed, $M(E_6)\oplus M(E_6)^*$ if $\bG=E_6$.

\begin{lemma} [{{\cite[Lemma 1.2]{craven2015un2}}}]
\label{lem:genericunipotent}
Suppose that $\bG=F_4,E_6,E_7$ with $p$ odd for $\bG=F_4$. Let $H$ be a finite subgroup of $\bG$ such that $H$ contains a non-trivial unipotent element whose action on a module $V$, one of $M(\bG)$, $M(E_6)\oplus M(E_6)^*$ if $\bG=E_6$, or $L(\bG)^\circ$ is generic. Then $u$ and $H$ are blueprints for $V$. In particular, $H$ is either strongly imprimitive or irreducible on $V$.
\end{lemma}
(The consequence follows from Proposition \ref{prop:blueprintissi}.)


Thus, if any subgroup $H$ of an exceptional algebraic group $\bG$ contains a unipotent element of order $p$ that is generic for either the minimal or adjoint module, then $H$ is either strongly imprimitive or $H$ acts irreducibly on this module. However, such subgroups are listed in \cite{liebeckseitz2004a}, so if $H$ does not appear on the list in \cite{liebeckseitz2004a} then $H$ is strongly imprimitive.

\medskip

For large primes, we will occasionally prove that $H$ stabilizes a unique $3$-dimensional submodule of $L(\bG)$, which must then be a subalgebra of the Lie algebra. If this $3$-dimensional submodule of $L(\bG)\downarrow_H$ is a summand then we may apply Proposition \ref{prop:sl2ifsplitoff} below and show that it is a copy of $\slf_2$, but if the $3$-dimensional submodule is not a summand then we cannot easily prove that it is an $\slf_2$, as it need not be simple. There is one case in particular where this occurs, which we refer to as a Serre embedding. These are embeddings of $\PSL_2(h+1)$ into an algebraic group in characteristic $h+1$, where $h$ is the Coxeter number of the group.

\begin{definition}\label{defn:serreembedding} Let $\bG$ be an exceptional algebraic group with Coxeter number $h$, and let $p=h+1$. A subgroup $H=\PSL_2(p)$ is a \emph{Serre embedding} if the following conditions hold:
\begin{enumerate}
\item on $L(\bG)$, $H$ stabilizes a unique $3$-dimensional subspace;
\item $H$ contains a regular unipotent element.
\end{enumerate}
\end{definition}

The $3$-dimensional subspace is in fact a subalgebra: the exterior square of a $3$-dimensional $kH$-submodule $W$ is $W^*\cong W$, and $\Hom_{kH}(\Lambda^2(W),L(E_8))$ is $1$-dimensional. From \cite[Lemma 1]{ryba2002}, $W$ is a Lie subalgebra of $L(E_8)$. Since this subspace need not (in fact, will not be) a summand of $L(E_8)\downarrow_H$, we cannot directly apply Proposition \ref{prop:sl2ifsplitoff} below.



\section{Blueprints and Element Orders}
\label{sec:blueprints}

The first result states that whether a semisimple class contains blueprints for a fixed Weyl module is independent of the characteristic of the underlying field. To prove this requires some of the theory of semisimple elements, for example \cite[Section 3.1.6]{litterickmemoir}. It also looks quite technical, but that is merely because we have to set up some bijection between characteristic $0$ and characteristic $p$, and also need to worry about the fact that the eigenvalues of a semisimple element on a Weyl module do not always determine the conjugacy class uniquely.

\begin{proposition}\label{prop:blueprintinvariant} Let $\bG_p$ and $\bG_0$ be simple, simply connected algebraic groups of the same type in characteristics $p$ and $0$ respectively. Let $V_p$ and $V_0$ denote the Weyl modules of a fixed weight for $\bG_p$ and $\bG_0$ respectively.

Let $a_1,\dots,a_d$ be integers. Let $n$ be a positive integer prime to $p$, and let $\theta_n$ and $\zeta_n$ be primitive $n$th roots of unity in $k$ and $\mathbb{C}$ respectively. Let $X_p$ and $X_0$ denote the set of elements of $\bG_p$ and $\bG_0$ with eigenvalues 
\[\{\theta_n^{a_i}\mid 1\leq i\leq d\}\quad \text{and}\quad \{\zeta_n^{a_i}\mid 1\leq i\leq d\}\]
on $V_p$ and $V_0$ respectively. The set $X_p$ consists solely of blueprints for $V_p$ if and only if the set $X_0$ consists solely of blueprints for $V_0$.
\end{proposition}
\begin{proof} Being a blueprint for a module is an invariant of the semisimple class, so we may assume that our elements lie in maximal tori $\bT_p$ and $\bT_0$ of $\bG_p$ and $\bG_0$ respectively. Choose bases of $V_p$ and $V_0$ so that $\bT_p$ and $\bT_0$ act diagonally. From the theory in \cite[Section 3.1.6]{litterickmemoir}, there is a bijection $f$ between $X_p\cap \bT_p$ and $X_0\cap \bT_0$, and a bijection between elements of $\bT_p$ of order $an$ for $a\geq 1$ powering to $x\in X_p\cap \bT_p$ and elements of $\bT_0$ of order $an$ powering to $f(x)$. Furthermore, this bijection preserves Brauer characters on $V_p$ and $V_0$, i.e., preserves eigenvalues under the assignment $\theta\mapsto \zeta$.

Suppose that $X_p$ consists of blueprints for $V_p$. Thus for each $x\in X_p\cap \bT_p$, there exist elements of arbitrarily large order in $\bT_p$ powering to $x$ and with the same number of distinct eigenvalues on $V_p$. Taking the corresponding elements of $\bT_0$, we find elements of arbitrarily large order $an$ for $a\geq 1$ in $\bT_0$ powering to $f(x)$. Hence each $f(x)$ is a blueprint for $V_0$.

The same argument would work as a converse if we could always choose $a$ to be prime to $p$. This is the case: if $x_0=f(x)$ lies in $\bT_0$ and the set of all elements of $\bT_0$ that stabilize all of the same subspaces of $V_0$ as $x_0$ forms a group of diagonal matrices, hence is a direct product of a torus and a finite abelian group by \cite[Theorem 16.2]{humphreyslag}. As a torus in characteristic $0$ contains a product of groups $\mathbb{\bar\Q}^\times$, and $\mathbb{\bar\Q}^\times$ contains elements of all orders, the result holds.
\end{proof}

We can also push being a blueprint for the minimal module of $F_4$ up into $E_6$ and $E_7$.

\begin{lemma}\label{lem:f4blueprintisblueprint} Let $\bG$ be $E_6$ or $E_7$, and let $x$ be a semisimple element of $\bG$ that lies in $F_4$. If $x$ is a blueprint for $M(F_4)$, then $x$ is a blueprint for $M(E_6)$, $M(E_6)\oplus M(E_6)^*$ and $M(E_7)$.
\end{lemma}
\begin{proof} The restrictions of the modules in question to $F_4$ have composition factors copies of $M(F_4)$ and trivial modules. Since $1$ is always an eigenvalue of any semisimple element of $F_4$ on $M(F_4)$, any element of $F_4$ with the same eigenspaces on $M(F_4)$ as $x$ also has the same eigenspaces on $M(E_6)$, $M(E_6)\oplus M(E_6)^*$ and $M(E_7)$. This completes the proof.
\end{proof}

The semisimple elements of $E_6$ that lie in $F_4$ are the real elements. Although the author has looked for a reference for this, beyond \cite[Theorem 3.1]{cohenwales1997}, which shows this only for order at most $7$, it does not appear to be easy to find explicitly. It follows almost immediately from results of Moody and Patera \cite{moodypatera1984}.

\begin{proposition}\label{prop:f4real} Let $\bG$ be the simply connected form of $E_6$. If $x$ is a real semisimple element of $\bG$ then $x$ is conjugate to an element of $F_4$.
\end{proposition}
\begin{proof} We use the results and notation of \cite[Section 4]{moodypatera1984}: if $x\in F_4$ is semisimple and its class corresponds to the Kac co-ordinates $(s_0,\dots,s_4)$, then the corresponding Kac co-ordinates in $E_6$ are $(s_0,s_1,s_2,s_3,s_2,s_1,s_4)$. By \cite[Proposition 5.3]{moodypatera1984}, a conjugacy class in $E_6$ is real if and only if its Kac co-ordinates have exactly this form, and hence all real semisimple classes of $E_6$ intersect $F_4$ non-trivially, as desired.
\end{proof}

If $\bG=E_7$ then $v(\bG)=75$ is fairly large, and in certain circumstances we can bring this down. Here is one such circumstance.

\begin{proposition}\label{prop:f4a4} Let $\bG$ be the simply connected form of $E_7$, and let $x$ be a semisimple element of $\bG$. If the $1$-eigenspace of $x$ on $M(E_7)$ has dimension at least $6$ then $x$ lies inside a conjugate of either an $F_4$ or $A_4$ subgroup. If in addition $o(x)>30$ then $x$ is a blueprint for $M(E_7)$.
\end{proposition}
\begin{proof} As in the proof of Proposition \ref{prop:numbersforE7}, we first place $x$ into the subgroup $A_7$. If $x$ centralizes a point on $\Lambda^2(M(A_7))$, then this requires one eigenvalue of $x$ on $M(A_7)$ to be the inverse of another. (In the notation of the proof of Proposition \ref{prop:numbersforE7}, $a_1=-a_2$.) This places $x$ into $A_1A_5$. However, by Lemma \ref{lem:e7stabs}, $x$ must lie in $E_6$ or $B_5$ (as if $x$ lies in a parabolic it lies in a Levi), whence $x$ lies in $E_6$. Since $x$ centralizes a $4$-space on $M(E_6)\oplus M(E_6)^*$, it must centralize a $2$-space $W$ on $M(E_6)$ (as it acts semisimply).

If $x$ lies in $F_4\leq E_6$ then we are done, so suppose not. From Lemma \ref{lem:e6stabs}, this means that $x$ cannot centralize an $F_4$-point, or a $B_4$-point, since $B_4\leq F_4$. In the notation of \cite{cohencooperstein1988}, this means that $W$ is a purely white $2$-space. By \cite[(P.3)]{cohencooperstein1988}, $W$ is unique up to action of $E_6$, and the stabilizer is an $A_1A_4$-parabolic of $E_6$, so the centralizer is an $A_4$-parabolic. Thus $x$ lies in $A_4$, as claimed.

If $x\in F_4$ and $o(x)>30$ then $x$ is a blueprint for $M(F_4)$ by Proposition \ref{prop:numbersforF4}, and hence a blueprint for $M(E_7)$ by Lemma \ref{lem:f4blueprintisblueprint}. On the other hand, if $x\in A_4$ then one uses Proposition \ref{prop:numbersforA4}. (The composition factors of $A_4$ on $M(E_7)$ are\[L(1000)^3,L(0100),L(0010),L(0001)^3,L(0000)^6\]
by \cite[Table 21]{thomas2016}, so the result may be used.) 
\end{proof}


Suppose we want to find the eigenvalues on $M(E_7)$ of semisimple elements of order $63$ inside $E_7$, which we will need to do when considering $\SL_2(64)$. There are too many to construct and store them all effectively, but we can take an element $x$ of order $21$ and consider all $3^7=2187$ elements $\hat x$ that cube to $x$ in a torus. Since we have the eigenvalues of all elements of order $21$, given a potential multiset of eigenvalues for an element $x$ of order $63$ in $E_7$, we take the eigenvalues of $x^3$, find all semisimple classes of elements of order $21$ with those eigenvalues, then consider all preimages of representatives of each of those classes. The eigenvalues of $x$ are valid for coming from $E_7$ if and only if one of those elements of order $21$ has a preimage with those values.

This idea to find the eigenvalues of elements of large composite order will be called the \emph{preimage trick} in the rest of this paper.


\section{Blueprints inside Subgroups of Type \texorpdfstring{$A_1$}{A1}}


We now prove that certain semisimple elements, and subgroups of the form $\SL_2(p^a)$ and $\PSL_2(p^a)$ of exceptional groups, are blueprints for a given module by examining the constituents of the restriction of the module to an $A_1$ subgroup containing the element or subgroup.

The first lemma deals with modules for the algebraic group $\SL_2$, and when the eigenspaces of semisimple elements match the weight spaces. Generalizing the idea of $p^a$-restricted, a highest weight module for $\SL_2$ is \emph{$n$-restricted} for some $n\in\N$ if its highest weight is $\lambda$ for $\lambda<n$.

\begin{lemma}\label{lem:restrictedsl2} Let $M$ be a module for $\SL_2$ with composition factors highest weight modules $L(\lambda_1),\dots,L(\lambda_r)$, arranged so that $\lambda_i\leq \lambda_{i+1}$. Let $\bT$ be a maximal torus of $\SL_2$, and let $x\in \bT$ be a semisimple element of order $n$. If $\lambda_r<n/2$ then the eigenvalues of $x$ on $M$ are the same as the weight spaces of $\bT$. In particular, $x$ is a blueprint for $M$.
\end{lemma}
\begin{proof} Since all maximal tori are conjugate, we may assume that $x$ is the matrix
\[ \begin{pmatrix}\zeta & 0\\0&\zeta^{-1}\end{pmatrix},\]
where $\zeta$ is a primitive $n$th root of $1$. The eigenvalues of $x$ on $L(1)$ are $\zeta,\zeta^{-1}$, and the eigenvalues of $x$ on $L(\lambda_i)$ are roots of unity $\zeta^{\pm j}$ for $0\leq j\leq \lambda_i$. If $\lambda_i<n/2$ for all $i$ then the eigenspaces of $x$ are simply the weight spaces of the $L(\lambda_i)$, and so $x$ and $\bT$ stabilize the same subspaces of $M$, thus $x$ is a blueprint for $M$.
\end{proof}

We will apply this lemma to $A_1$ subgroups of algebraic groups. We often will end up with composition factors that do not precisely satisfy the hypotheses of this lemma though: if one composition factor has slightly larger highest weight, then although the eigenspaces do not correspond to weight spaces, with some weight spaces being merged, these all take place within one composition factor of the module, and so the finite subgroup $A_1(q)$ of the $A_1$ is still a blueprint for the module in question, even if the element of order $n$ is not.

\begin{lemma}\label{lem:q/2restricted} Let $\bG$ be the simply connected form of an exceptional algebraic group, and let $\bX$ be a positive-dimensional subgroup of $\bG$ of type $A_1$. Let $x$ be a semisimple element of $\bX$ of order $n$. Let $M$ be a module for $\bG$.
\begin{enumerate}
\item\label{lemi:q2resa} If the composition factors of $\bX$ on $M$ are $n/2$-restricted then $x$ and a maximal torus $\bT$ containing $x$ stabilize the same subspaces of $M$, so that $x$ is a blueprint for $M$.
\item\label{lemi:q2resb} Suppose that the highest weights of $\bX$ on $M$ are $\lambda_1,\dots,\lambda_r$, with $\lambda_i\leq \lambda_{i+1}$, and let $H=A_1(q)$ be a finite subgroup of $\bX$ containing $x$. If $\lambda_{r-1}+\lambda_r<n$ then $H$ and $\bX$ stabilize the same subspaces of $M$, so that $H$ is a blueprint for $M$.
\end{enumerate}
\end{lemma}
\begin{proof} The first part follows immediately from Lemma \ref{lem:restrictedsl2}, so we concentrate on the second statement. Letting $\bT$ be a maximal torus of $\bX$ containing $x$, if $\lambda$ and $\mu$ are two weights of $\bT$ on $M$ that are equal when taken modulo $n$ (i.e., yield the same eigenvalue for the action of $x$), then $\lambda$ and $\mu$ differ by a multiple of $n$. By assumption on the $\lambda_i$, since $\lambda-\mu\geq n$, both $\lambda$ and $\mu$ must be weights for the composition factor $L(\lambda_r)$, since if $\lambda$ is a weight for one of the other $L(\lambda_i)$ then it lies between $-\lambda_i$ and $+\lambda_i$, and cannot differ by $n$ from any other weight for any other $\lambda_j$.

Let $N$ be any $kH$-submodule of $M$. If $N$ does not contain the factor $L(\lambda_r)$ then the eigenvectors of $x$ on $N$ all come from weight vectors for $\bT$, by the previous paragraph, and so $\bT$ stabilizes $N$. If $N$ contains $L(\lambda_r)$, then $\bT$ also stabilizes $N$ by taking duals: $\bT$ stabilizes the submodule $\Ann(N)$ of $M^*$, which is isomorphic to $(M/N)^*$. Thus $\bT$ stabilizes every $H$-submodule of $M$, and so $\gen{\bT,H}=\bX$ and $H$ stabilize the same subspaces of $M$, as claimed.
\end{proof}


\section{Traces of Modules for \texorpdfstring{$\PGL_2$}{PGL2}}
\label{sec:pgl}
For this section $p$ is odd. Here we produce a technical result about extending simple modules for $\PSL_2(p^a)$ to $\PGL_2(p^a)$, and the traces and eigenvalues of the elements on such an extension.

There are two extensions of any simple module from $\PSL_2(p^a)$ to $\PGL_2(p^a)$. We will give a way of telling these apart if the dimension of the simple module is odd, which is all that we need in what follows.

If $L(i)$ is a simple module for $\PSL_2(p^a)$ of odd dimension, then of the two extensions of $L(i)$ to $\PGL_2(p^a)$, for one all defining matrices have determinant $1$ and for the other half have determinant $-1$: to see this, note that all elements in $\PSL_2(p^a)$ act with determinant $1$, and the non-trivial $1$-dimensional representation acts like $-1$ for elements outside of $\PSL_2(p^a)$, so a given extension and its product with this $1$-dimensional representation give us the two cases. Write $L(i)^+$ for the module for $\PGL_2(p^a)$ for which all matrices have determinant $+1$, and $L(i)^-$ for the other extension. This notation will be used in the proof of the next lemma.

\begin{lemma}\label{lem:pglnotappearing} Let $p$ be an odd prime and $a\geq 1$ an integer. Let $M$ be a simple module for $H=\PGL_2(p^a)$ with Brauer character $\phi$, and let $g$ be an element of order $p^a\pm 1$ in $H$. Let $t$ be an involution in $\PSL_2(p^a)$, and let $h$ be the involution in $\gen g$.
\begin{enumerate}
\item There are two conjugacy classes of involutions in $H$. If $o(g)$ is twice an odd number then $t$ and $h$ are representatives of these two classes, and otherwise $t$ and $h$ are conjugate.
\item If $\dim(M)$ is even then $\phi(t)=\phi(h)=0$.
\item If $\dim(M)$ is odd, then the dimensions of the $(+1)$-eigenspace and $(-1)$-eigenspace of the action of $g$ differ by $1$.
\item If $\dim(M)$ is odd, then $\phi(t)=\pm\phi(h)$. Furthermore, if $+1$ is not an eigenvalue of $g$ on $M$, then $\phi(t)=\phi(h)$ if and only if $t$ and $h$ are conjugate. If $-1$ is not an eigenvalue of $g$ on $M$ then $\phi(t)=\phi(h)$.
\end{enumerate}
\end{lemma}
\begin{proof}
\begin{enumerate}
\item That $H$ has two classes of involutions is well known, and one is a class of complements, the other is in $\PSL_2(p^a)$. Thus the second statement follows easily.
\item We use Steinberg's tensor product theorem, lifting all modules to $\GL_2(p^a)$: $M$ has even dimension if and only if, as a tensor product, at least one of the factors has even dimension, and the Brauer character is $0$ for a given element if and only if one of the factors has Brauer character $0$ for the same element. Thus we need to check this for the symmetric powers of the natural module $S^i(M')$ for $0\leq i\leq p-1$ (where $M'$ is the natural module for $\GL_2$), where it is trivial to see that the trace of an involution is $0$ on even-dimensional modules and $\pm 1$ on modules of odd dimension.

\item Since $\dim(M)$ is odd and $M$ is self-dual, of course one of $\pm 1$ is an eigenvalue for the action of $g$ on $M$, and the dimensions of the $(+1)$- and $(-1)$-eigenspaces must differ by an odd number. It is an easy exercise to compute the eigenvalues of $g$ on the Steinberg module $L(p^a-1)^\pm$ for $\PGL_2(p^a)$, and we see that these are all distinct if $g$ has order $p^a+1$, and if $g$ has order $p^a-1$ then $\pm 1$ appears twice and $\mp1$ appears once.

For other modules, from the definition of the Steinberg module as a tensor product of twists of the $p$-restricted module $L(p-1)^\pm$, and the fact that the eigenvalues of $g$ on $L(i)^\pm$ all appear in $L(p-1)^\pm$, we see that the eigenvalues of $g$ on any simple module appear in the eigenvalues of $g$ on the Steinberg. Thus the result holds since the sum of the dimensions of the $(+1)$- and $(-1)$-eigenspaces must be odd.

\item Return to $\PGL_2(p^a)$, and suppose that $t$ and $h$ are not conjugate, so that $g$ has twice odd order. As we saw above, for a $p$-restricted module $L(i)^\pm$ for $0\leq i\leq p-1$ an even integer, the Brauer character values of $L(i)^+$ on $t$ and $h$ have the same sign, and the Brauer character values of $L(i)^-$ on $t$ and $h$ have opposite signs. Notice that $+1$ is an eigenvalue of $M$ if and only if there are an even number of minus-type modules in the tensor decomposition, and this happens if and only if $\phi(t)=\phi(h)$, as needed.
\end{enumerate}
\end{proof}

Using this, the following result is now clear.

\begin{corollary}\label{cor:sl2nopgl} Let $p$ be an odd prime and $a\geq 1$ an integer. Let $\bG$ be the simply connected form of $E_7$, and let $H$ be a copy of $\SL_2(p^a)$ in $\bG$ with $Z(\bG)=Z(H)$. Suppose that $g$ is an element of $\bG$ such that $o(g)=p^a\pm 1$ is twice an odd number, and $-1$ is not an eigenvalue for the action of $g$ on $L(E_7)$. Then the group $\bar H=\gen{H,g}$ does not satisfy $\bar H/Z(H)=\PGL_2(p^a)$.
\end{corollary}
\begin{proof} Suppose that $\bar H/Z(H)=\PGL_2(p^a)$. Let $t$ be an element of $H$ that is an involution in $H/Z(H)$, so $o(t)=4$. The trace of $t$ on $L(E_7)$ is $-7$ or $25$, depending on the class of $t$ in $\bG$. The involution $h$ in $\gen g$ has trace $5$ on $L(E_7)$, since it is an involution in $\bG$ rather than $\bG/Z(\bG)$. We now show that $h$ and $t$ must in fact have the same trace, which is a contradiction. By Lemma \ref{lem:pglnotappearing}, any even-dimensional composition factors of $L(E_7)\downarrow_H$ yield trace $0$ for both $t$ and $h$, and they have the same trace on odd-dimensional composition factors since $-1$ is not an eigenvalue of $g$ on $L(E_7)$. Thus the trace of $t$ and $h$ on $L(E_7)$ is the same, but this is a contradiction.
\end{proof}

This is how we will use Corollary \ref{cor:sl2nopgl}: suppose that $H\cong \SL_2(p^a)$ lies inside the simply connected form $\bG$ of $E_7$ with $Z(\bG)=Z(H)$. We find some element $x\in \bG$ such that $x$ and $H$ both stabilize some proper subspace $W$ of either $M(E_7)$ or $L(E_7)$, so that $\gen{H,x}$ is not of the same type as $\bG$. If $-1$ is not an eigenvalue of $x$ on $L(E_7)$ then $\gen{H,x}$, modulo $Z(\bG)$, is not $\PGL_2(p^a)$ either. If the composition factors of $L(E_7)\downarrow_H$ are not invariant under a field automorphism of $H$, then $x$ cannot induce a field automorphism on $H$, and therefore $\gen{H,x}$ is not almost simple modulo $Z(\bG)$ either. If, in addition, $H$ is a maximal member of $\mathscr P$, then we apply Proposition \ref{prop:maximalnotinP} to see that $H$ is Lie imprimitive. Furthermore, if we chose $W$ so that it is stable under $N_{\Aut^+(\bG)}(H)$, or our element $x$ stabilizes all submodules in the $N_{\Aut^+(\bG)}(H)$-orbit of $W$, then $H$ is also strongly imprimitive.

\section{The Graph Automorphism of \texorpdfstring{$F_4$}{F4}}

In this short section we describe how semisimple elements of odd order in $F_4$ react to the graph automorphism in characteristic $2$. Since the graph automorphism $\tau$ does not stabilize the minimal module $M(F_4)$, and $L(F_4)$ has composition factors $M(F_4)$ and $M(F_4)^\tau$, we can see the effect of the graph automorphism on semisimple classes by taking the eigenvalues of an element $x$ on $L(F_4)$ and removing those from $M(F_4)$.

Since the graph automorphism squares to a field automorphism, however, it is slightly more complicated to understand those classes that are left invariant under a graph automorphism, since we need to check whether the eigenvalues of $x^\tau$ and $x^i$ match for some $i$, rather than whether the eigenvalues of $x$ and $x^\tau$ match. This is still not difficult using a computer, however; we give two special cases, where a conjugacy class is stable under the graph automorphism (up to powers) and where the classes have integral traces.

\begin{lemma} Let $k$ be a field of characteristic $2$. Let $x$ be a semisimple element in $G=F_4(k)$ such that $x^\tau$ is conjugate to a power of $x$. If $x$ has order at most $9$, then a power of $x$ has trace on $M(F_4)$ given below.

\begin{center}
\begin{tabular}{cc}
\hline $o(x)$ & Possible traces on $M(F_4)$
\\\hline $3$ & $-1$
\\ $5$ & $1$
\\ $7$ & $4(\zeta_7+\zeta_7^{-1})+3(\zeta_7^2+\zeta_7^{-2})+5$, $-(\zeta_7+\zeta_7^{-1})$
\\ $9$ & $2-3(\zeta_9+\zeta_9^{-1})$ 
\\\hline
\end{tabular}
\end{center}
\end{lemma}


\begin{lemma}\label{lem:swappingintegralf4} Let $k$ be a field of characteristic $2$. Let $x$ be a semisimple element in $G=F_4(k)$ such that the trace of both $x$ and $x^\tau$ is an integer, and $x$ and $x^\tau$ are not conjugate. If $x$ has order at most $9$, then the traces of $x$ and $x^\tau$ are as below, where we give $x$ up to graph automorphism.

\begin{center}
\begin{tabular}{ccc}
\hline $o(x)$ & Trace of $x$ on $M(F_4)$ & Trace of $x^\tau$ on $M(F_4)$
\\\hline $3$ & $8$ & $-1$
\\ $5$ & None & None
\\ $7$ & $-2$ & $5$ 
\\ $9$ & $-1$ ($x^3$ has trace $-1$) & $2$ ($x^3$ has trace $-1$)
\\\hline
\end{tabular}
\end{center}
\end{lemma}

\section{Rank-1 Subalgebras of the Lie Algebra}
\label{sec:sl2subalgebra}

In this section we consider subalgebras of $L(\bG)$, specifically $\slf_2$-subalgebras. The stabilizers of $\slf_2$-subalgebras will be shown to be positive dimensional if $p$ is not too small. Thus if a subgroup $H$ of $\bG$ stabilizes a unique $3$-space on $L(\bG)$, and this is an $\slf_2$-subalgebra, then $H$ is Lie imprimitive, and must be strongly imprimitive via Proposition \ref{prop:intersectionstabilizers}, since the subspace is unique.

To begin with, we prove a proposition that gives us a criterion for a subgroup $H$ to stabilize an $\slf_2$-subalgebra in the first place. This proposition is a restatement of results of Ryba from \cite{ryba2002}, particularly Lemma 10 from that paper.

\begin{proposition}\label{prop:sl2ifsplitoff} Let $V$ be a $3$-dimensional subspace of $L(\bG)$, and let $H$ be a subgroup of $\bG$ such that $HZ(\bG)/Z(\bG)=\PSL_2(p^a)$ for some $p\geq 5$. If $V$ is $H$-stable and a complement for $V$ is also $H$-stable (i.e., $V$ is a summand of $L(\bG)\downarrow_H$), and $\Hom_{kH}(V,L(\bG))$ is $1$-dimensional (i.e., there are no other submodules of $L(\bG)\downarrow_H$ isomorphic to a quotient of $V$) then $V$ is a subalgebra of $L(\bG)$ isomorphic to $\slf_2$.
\end{proposition}
\begin{proof} As $\Hom_{kH}(V,L(\bG))$ is $1$-dimensional, $V$ is a non-trivial module, and therefore $V$ is isomorphic to the module $3_i$ for some $i$ for $H/Z(H)$. In particular, it is self-dual.

Suppose that $L(\bG)\downarrow_H$ has a unique submodule isomorphic to $V$, and that this is a summand, so that the quotient $L(\bG)\downarrow_H/V$ has no quotient isomorphic to $V^*\cong V$. By \cite[Lemma 6]{ryba2002}, we have that $V$ possesses a non-singular trace form, and then we apply Block's theorem \cite{block1962} to see that $V$ is a simple Lie algebra of type $\slf_2$.
\end{proof}

In order to use this proposition, we need to know something about the $\slf_2$-subalgebras of the Lie algebras of exceptional groups. The following is a theorem of Stewart and Thomas \cite[Theorem 1.2]{stewartthomas2018}, specialized to the case of $\bG=E_6,E_7,E_8$, for use in this paper and a later one on $\SL_2$-subgroups of $E_8$.

\begin{theorem}\label{thm:sl2subalgebra}
Let $\bG=E_6$ and $p\geq 7$, or $\bG=E_7,E_8$ and $p\geq 11$. The classes of $\slf_2$-subalgebras of $L(\bG)$ are in one-to-one correspondence with the nilpotent orbits of $L(\bG)$, with a bijection being realized by sending an $\slf_2$-subalgebra to the nilpotent orbit of largest dimension intersecting it non-trivially.
\end{theorem}

To prove \cite[Theorem 1.2]{stewartthomas2018}, representatives for $\slf_2$-triples $(e,h,f)$ for each class of $\slf_2$-subalgebra were constructed using a computer and the `Tools' referred to in \cite[Proof of Theorem 1.2]{stewartthomas2018}. David Stewart has kindly shared this computer file, and so it was possible to compute the Jordan block structures of the nilpotent elements $f$ in each triple. If $e^{[p]}=0$ then $e$ and $f$ lie in the same orbit, but if $e^{[p]}\neq 0$ then the orbits of $e$ and $f$ are different, $f^{[p]}=0$, and the precise orbit of $f$ for $p\geq 5$ is given in Tables \ref{t:sl2classesE6}, \ref{t:sl2classesE7} and \ref{t:sl2classesE8}. This yields the following corollary.

\begin{table}
\begin{center}
\begin{tabular}{cccc}
\hline Class & $p=5$ & $p=7$ & $p=11$
\\\hline$D_{4}$&$3A_{1}$&&
\\$A_{5}$&$A_{3}$&&
\\$D_{5}(a_{1})$&$A_{2}+A_{1}$&&
\\$E_{6}(a_{3})$&$A_{3}+A_{1}$&&
\\$D_{5}$&$A_{3}$&$A_{3}+A_{1}$&
\\$E_{6}(a_{1})$&$2A_{2}+A_{1}$&$A_{5}$&
\\$E_{6}$&$A_{2}+2A_{1}$&$2A_{2}+A_{1}$&$A_5$
\\ \hline
\end{tabular}
\end{center}
\caption{Second nilpotent class intersecting a non-restricted $\slf_2$-subalgebra of $L(E_6)$ for $p\geq 5$}
\label{t:sl2classesE6}
\end{table}

\begin{table}\begin{center}
\begin{tabular}{cccccc}
\hline Class & $p=5$ & $p=7$ & $p=11$ & $p=13$ & $p=17$
\\\hline $D_{4}$&$(3A_{1})'$&&&&
\\$(A_{5})''$&$A_{3}$&&&&
\\$D_{4}+A_{1}$&$4A_{1}$&&&&
\\$D_{5}(a_{1})$&$A_{2}+A_{1}$&&&&
\\$(A_{5})'$&$A_{3}$&&&&
\\$A_{5}+A_{1}$&$(A_{3}+A_{1})'$&&&&
\\$D_{5}(a_{1})+A_{1}$&$A_{2}+2A_{1}$&&&&
\\$D_{6}(a_{2})$&$D_{4}(a_{1})+A_{1}$&&&&
\\$E_{6}(a_{3})$&$(A_{3}+A_{1})'$&&&&
\\$D_{5}$&$A_{3}$&$(A_{3}+A_{1})'$&&&
\\$E_{7}(a_{5})$&$A_{3}+A_{2}$&&&&
\\$A_{6}$&$A_{2}+2A_{1}$&&&&
\\$D_{5}+A_{1}$&$(A_{3}+A_{1})'$&$A_{3}+2A_{1}$&&&
\\$D_{6}(a_{1})$&$A_{3}+2A_{1}$&$D_{4}(a_{1})+A_{1}$&&&
\\$E_{7}(a_{4})$&$D_{4}(a_{1})+A_{1}$&$A_{3}+A_{2}$&&&
\\$D_{6}$&$A_{3}$&$A_{3}+2A_{1}$&&&
\\$E_{6}(a_{1})$&$2A_{2}+A_{1}$&$(A_{5})'$&&&
\\$E_{6}$&$A_{2}+2A_{1}$&$2A_{2}+A_{1}$&$(A_{5})'$&&
\\$E_{7}(a_{3})$&$(A_{3}+A_{1})'$&$D_{4}(a_{1})+A_{1}$&&&
\\$E_{7}(a_{2})$&$2A_{2}+A_{1}$&$A_{3}+2A_{1}$&$D_{6}(a_{2})$&&
\\$E_{7}(a_{1})$&$A_{2}+2A_{1}$&$(A_{5})'$&$D_{6}$&$D_6(a_1)$&
\\$E_{7}$&$A_{4}+A_{2}$&$A_{6}$&$A_{5}+A_{1}$&$D_5+A_1$&$D_6$
\\ \hline
\end{tabular}
\end{center}
\caption{Second nilpotent class intersecting a non-restricted $\slf_2$-subalgebra of $L(E_7)$ for $p\geq 5$}
\label{t:sl2classesE7}
\end{table}


\begin{table}\begin{center}
\begin{tabular}{ccccc}
\hline Class & $p=5$ & $p=7$ & $p=11$ & $p=13$
\\\hline $D_{4}$&$3A_{1}$&&&
\\$A_{5}$&$A_{3}$&&&
\\$D_{4}+A_{2}$&$A_{2}+3A_{1}$&&&
\\$E_{6}(a_{3})$&$A_{3}+A_{1}$&&&
\\$D_{5}$&$A_{3}$&$A_{3}+A_{1}$&&
\\$A_{5}+A_{1}$&$A_{3}+A_{1}$&&&
\\$D_{5}(a_{1})+A_{2}$&$2A_{2}+A_{1}$&&&
\\$E_{6}(a_{3})+A_{1}$&$A_{3}+2A_{1}$&&&
\\$D_{5}+A_{1}$&$A_{3}+A_{1}$&$A_{3}+2A_{1}$&&
\\$E_{8}(a_{7})$&$A_4+A_3$&&&
\\$A_{6}+A_{1}$&$A_{2}+3A_{1}$&&&
\\$E_{6}(a_{1})$&$2A_{2}+A_{1}$&$A_{5}$&&
\\$D_{5}+A_{2}$&$A_{3}+A_{2}$&$A_{3}+A_{2}+A_{1}$&&
\\$E_{6}$&$A_{2}+2A_{1}$&$2A_{2}+A_{1}$&$A_{5}$&
\\$D_{7}(a_{2})$&$2A_{3}$&$A_{4}+A_{1}$&&
\\$A_{7}$&$2A_{2}+A_{1}$&$A_{5}$&&
\\$E_{6}(a_{1})+A_{1}$&$2A_{2}+2A_{1}$&$A_{5}+A_{1}$&&
\\$E_{7}(a_{3})$&$A_{3}+A_{1}$&$D_{4}(a_{1})+A_{1}$&&
\\$E_{8}(b_{6})$&$D_{4}(a_{1})+A_{1}$&$E_{7}(a_{5})$&&
\\$D_{7}(a_{1})$&$A_{3}+2A_{1}$&$A_{3}+A_{2}$&&
\\$E_{6}+A_{1}$&$A_{2}+3A_{1}$&$2A_{2}+2A_{1}$&$A_{5}+A_{1}$&
\\$E_{8}(a_{6})$&$2A_{3}$&$A_{4}+2A_{1}$&&
\\$D_{7}$&$A_{2}+3A_{1}$&$A_{5}$&$D_{5}+A_{1}$&
\\$E_{8}(b_{5})$&$2A_{2}+2A_{1}$&$D_{4}(a_{1})+A_{1}$&$E_{7}(a_{5})$&
\\$E_{7}(a_{1})$&$A_{2}+2A_{1}$&$A_{5}$&$D_{6}$&$D_{6}(a_{1})$
\\$E_{8}(a_{5})$&$2A_{2}+A_{1}$&$E_{6}(a_{3})+A_{1}$&$E_{7}(a_{4})$&
\\$E_{8}(b_{4})$&$A_{2}+3A_{1}$&$A_{5}+A_{1}$&$E_{7}(a_{3})$&$E_{7}(a_{4})$
\\$E_{8}(a_{4})$&$A_{4}+A_{3}$&$A_{5}$&$D_{6}(a_{2})$&$E_{7}(a_{3})$
\\$E_{8}(a_{3})$&$A_{4}+A_{2}+A_{1}$&$A_{6}+A_{1}$&$E_{6}(a_{3})+A_{1}$&$D_{6}(a_{1})$
\\$E_{8}(a_{2})$&$2A_{3}$&$A_{4}+A_{3}$&$A_{5}+A_{1}$&$D_{7}$
\\$E_{8}(a_{1})$&$2A_{2}+2A_{1}$&$A_{4}+A_{2}+A_{1}$&$D_{5}(a_{1})+A_{2}$&$A_{7}$
\\$E_{8}$&$A_{3}+A_{2}+A_{1}$&$A_{3}+A_{2}+A_{1}$&$A_{4}+A_{3}$&$A_{6}+A_{1}$
\\ \hline
\\ \hline Class & $p=17$ & $p=19$ & $p=23$ & $p=29$
\\ \hline $E_8(a_3)$ & $E_7(a_3)$&&&
\\ $E_8(a_2)$ & $E_7(a_1)$&$E_7(a_2)$&&
\\$E_{8}(a_{1})$&$D_{7}$&$E_{7}$&$E_{7}(a_{1})$&
\\$E_{8}$&$A_{7}$&$E_{6}+A_{1}$&$D_{7}$&$E_{7}$
\\ \hline
\end{tabular}
\end{center}
\caption{Second nilpotent class intersecting a non-restricted $\slf_2$-subalgebra of $L(E_8)$ for $p\geq 5$. (Missing classes, $D_4+A_1$, $D_5(a_1)$, $D_5(a_1)+A_1$, $D_6(a_2)$, $E_7(a_5)$, $A_6$, $D_6(a_1)$, $E_7(a_4)$, $D_6$, $E_7(a_2)$ and $E_7$, are exactly as in Table \ref{t:sl2classesE7})}
\label{t:sl2classesE8}
\end{table}

\begin{corollary}\label{cor:sl2coxeter-1} Let $\bG=E_6$ and $p\geq 7$, or $\bG=E_7,E_8$ and $p\geq 11$. Let $H\cong\PSL_2(p^a)$ be a subgroup of $\bG/Z(\bG)$. If $H$ stabilizes an $\slf_2$-subalgebra $\mathfrak h$ of $L(\bG)$, then $\mathfrak{h}$ is restricted and $H$ is Lie imprimitive. If, in addition, $H$ stabilizes a unique $3$-space on $L(\bG)$ then $H$ is strongly imprimitive.
\end{corollary}
\begin{proof} Since there is a unique conjugacy class of subgroups $\PSL_2(p^a)$ inside $\PSL_2$, we see that because the standard $\PSL_2(p^a)$ inside $\PSL_2$ swaps $e$ and $f$ in an $\slf_2$-triple $(e,h,f)$ for $\mathfrak{h}$, thus $H$ must swap the two nilpotent orbits of $\mathfrak{h}$. From the discussion above this result, if $\mathfrak{h}$ is not restricted then $e$ and $f$ lie in different nilpotent orbits of $L(\bG)$, so $\mathfrak{h}$ must be restricted.

Now we argue exactly as in \cite[Proof of Theorem 1.6]{stewartthomas2018}, using \cite[Proposition 4.1]{seitz2000} to find $\bX$ a good $A_1$ in $\bG$ that stabilizes $\mathfrak{h}$. Hence $\gen{H,\bX}$ is positive dimensional and stabilizes $\mathfrak h$, so $H$ is Lie imprimitive. If $H$ stabilizes a unique $3$-space on $L(\bG)$ then Proposition \ref{prop:intersectionstabilizers} shows that $\bX$ is $N_{\Aut^+(\bG)}(H)$-stable, and therefore $H$ is strongly imprimitive.
\end{proof}

\endinput

